Likelihood Ratio Exponential Families

The exponential family is well known in machine learning and statistical physics as the maximum entropy distribution subject to a set of observed constraints, while the geometric mixture path is common in MCMC methods such as annealed importance sampling. Linking these two ideas, recent work has interpreted the geometric mixture path as an exponential family of distributions to analyze the thermodynamic variational objective (TVO). We extend these likelihood ratio exponential families to include solutions to rate-distortion (RD) optimization, the information bottleneck (IB) method, and recent rate-distortion-classification approaches which combine RD and IB. This provides a common mathematical framework for understanding these methods via the conjugate duality of exponential families and hypothesis testing. Further, we collect existing results to provide a variational representation of intermediate RD or TVO distributions as a minimizing an expectation of KL divergences. This solution also corresponds to a size-power tradeoff using the likelihood ratio test and the Neyman Pearson lemma. In thermodynamic integration bounds such as the TVO, we identify the intermediate distribution whose expected sufficient statistics match the log partition function.

==> sections/app/displaced_eq.tex <==

% \subsection{Displaced Equilibrium Construction}
% \begin{figure}
% \includegraphics[width=.5\textwidth]{figs/bercher.pdf}
% \end{figure}

% \citet{bercher2012simple} consider a `displaced equilibrium' problem, where force is applied to displace an initial state $\pi_0$ by a given relative entropy $D_{KL}[\, r \, || \pi_0 ] = R$.  The system is then `attracted' toward a second distribution $\pi_1$ to obtain a new equilibrium.
% \begin{align}
%      \mathcal{F}(R) = \min_{r} & \, D_{KL}[r(\omega) || \pi_1 (\omega)] \quad \text{subj. } \quad D_{KL}[r(\omega) || \pi_0 (\omega)] = R \\ 
%      = \max \limits_{\lambda} \min \limits_{r} &  \, D_{KL}[r(\omega) || \pi_1 (\omega)] + \lambda \big( D_{KL}[r(\omega) || \pi_0 (\omega)] - R \big) \label{eq:fr}
% \end{align}
% % \begin{align*}
% %     \min_[r] D_{KL}[r(\omega) || \pi_1 (\omega)] \quad \text{subj. } \quad D_{KL}[r(\omega) || \pi_0 (\omega)] = R
% % \end{align*}
% As derived in \cref{app:fr_optimum}, the solution to this optimization is given by
% \begin{align}
%     r^{*}(\omega) := \pi_{\alpha}(\omega) = \frac{\pi_0 (\omega)^{1-\alpha}{\pi_1 (\omega)^{\alpha}}}{\exp \{ \log \mathbb{E}_{\pi_0} \frac{\pi_1^{\alpha}}{\pi_0^{\alpha}} \} } = \frac{\tilde{\pi}_{\alpha} (\omega)}{ \exp \psi_{\alpha}} \label{eq:r_opt}
% \end{align}
% where $\alpha = \frac{1}{1+\lambda}$ and $\lambda = \frac{1-\alpha}{\alpha} $ is the Lagrange multiplier enforcing the constraint in \eqref{eq:fr}.  Plugging this solution into the Lagrangian,
% \begin{align*}
%     \mathcal{F}(R) &= D_{KL}[\pi_{\alpha}(\omega) || \pi_1 (\omega)] + \frac{1-\alpha}{\alpha} D_{KL}[\pi_{\alpha}(\omega) || \pi_0 (\omega)] - \frac{1-\alpha}{\alpha} \, R \\
%     &= \frac{1}{\alpha} \bigg( \alpha \, \psi (1) + (1-\alpha) \, \psi (0) - \psi (\alpha) \bigg) -  \frac{1-\alpha}{\alpha} \, R
% \end{align*}
% with $\psi (\alpha)$ denoting the partition function as in \eqref{eq:r_opt} and detailed derivations in \cref{app:fr_optimum}.  
% % \footnote{Note, for distributions without a path exponential family \cite{brekelmans2019tvo}, we consider $D_{KL}[\pi_{\alpha}(\omega) || \pi_1 (\omega)] = D_{\psi}[ \pi_1 (\omega) || \pi_{\alpha}(\omega) ] = \psi_1 - \psi_{\alpha} - (1-\alpha) \eta_{\alpha}$ with $\eta_{\alpha} = \frac{\partial}{\partial \alpha} \psi_{\alpha}$.}
% It can also be shown that the Renyi divergence between members of an exponential family corresponds to a gap in Jensen's inequality as above, so that $(1-\alpha) D_{\alpha}[\pi_1 || \pi_0] = \alpha \, \psi (1) + (1-\alpha) \, \psi (0) - \psi (\alpha)$.  Thus, minimization of $\mathcal{F}(R)$ amounts to minimizing a Renyi divergence, with order $\alpha$ determined by the constraint value $R$.  \citet{bercher2012simple} also show that minimizing $\mathcal{F}(R)$ also corresponds to minimizing $D_{KL}[\pi_1 || \pi_0]$ or the symmetrized KL divergence when the constraint is filled.


% \section{Optimum of $\mathcal{F}(R)$}\label{app:fr_optimum}
% \begin{align*}
%      \mathcal{F}(R) &= \min_{r} D_{KL}[r(\omega) || \pi_1 (\omega)] \quad \text{subj. } \quad D_{KL}[r(\omega) || \pi_0 (\omega)] = R \\
%      \implies 0 &=\frac{d}{d \lambda} \bigg( \mathbb{E}_{r} \log r(\omega) - \mathbb{E}_{r} \log \pi_1 (\omega) + \lambda ( D_{KL}[r(\omega) || \pi_0 (\omega)] - R )  \bigg) \\
%      &= 1 + \log r(\omega) - \log \pi_1 (\omega) + \lambda +  \lambda \log r(\omega) - \lambda \log \pi_0(\omega) - \lambda R \\
%      \implies r(\omega) &= \frac{\pi_0(\omega)^{\frac{\lambda}{1+\lambda}} \pi_1(\omega)^{\frac{1}{1+\lambda}}}{\int \pi_0(\omega)^{\frac{\lambda}{1+\lambda}} \pi_1(\omega)^{\frac{1}{1+\lambda}} d\omega} \\
% \end{align*}
% Letting $\frac{1}{1+\lambda} = \alpha$, we obtain $r(\omega) &= \frac{\pi_0(\omega)^{1-\alpha} \pi_1(\omega)^{\alpha}}{\exp \{ \psi(\alpha) \} }$.

% We use the notation of the path exponential family \cite{brekelmans2019tvo}, with natural parameter $\alpha$, base distribution $\pi_0(\omega)$, and $T(\omega) = \log \pi_1 / \pi_0$.  This induces a log partition $\psi(\alpha) = \log \int \pi_0(\omega)^{1-\alpha} \pi_1(\omega)^{\alpha} d\omega$, with a Bregman divergence $D_{\psi}[\pi_0 || \pi_{\alpha}] = D_{KL}[\pi_{\alpha}  || \pi_0]$.
% \begin{align*}
%     \mathcal{F}(R) &= D_{KL}[\pi_{\alpha}(\omega) || \pi_1 (\omega)] + \frac{1-\alpha}{\alpha} D_{KL}[\pi_{\alpha}(\omega) || \pi_0 (\omega)] - \frac{1-\alpha}{\alpha} \, R \\
%     &= \, \, \, D_{\psi} \, [\pi_1 (\omega) || \pi_{\alpha}(\omega) ] + \frac{1-\alpha}{\alpha} D_{KL}[ \pi_0 (\omega)  ||  \pi_{\alpha}(\omega) ] - \frac{1-\alpha}{\alpha} \, R \\
%     &= \psi(1) - \psi(\alpha) - (1 - \alpha) \, \eta_{\alpha} + \frac{1-\alpha}{\alpha} \psi(0) -\frac{1-\alpha}{\alpha} \psi(\alpha) - \frac{1-\alpha}{\alpha}  (0 - \alpha) \, \eta_{\alpha} - \frac{1-\alpha}{\alpha} \, R \\
%     &= \psi(1) + \frac{1-\alpha}{\alpha} \psi(0) - \frac{1}{\alpha} \, \psi(\alpha) - \frac{1-\alpha}{\alpha} \, R \\
%     &= \frac{1}{\alpha} \big( \alpha \, \psi(1) + (1-\alpha) \, \psi(0) - \psi(\alpha) - (1-\alpha) \, R \big) \\
%     &= \frac{(1-\alpha)}{\alpha} D_{\alpha}[\pi_1 || \pi_0 ] - \, R \\
%     &= \textbf{double check}
% %  &= \psi_1 - \psi_{\alpha} - (1 - \alpha) \eta_{\alpha} + \frac{1-\alpha}{\alpha} \psi_0 -\frac{1-\alpha}{\alpha} \psi_{\alpha} - \frac{1-\alpha}{\alpha}  (0 - \alpha) \eta_{\alpha} - \frac{1-\alpha}{\alpha} \, R
% \end{align*}

==> sections/app/noneq.tex <==
\section{Non-Equilibrium Thermodynamics}
In this section, we draw connections with physical simulations of thermodynamic systems \cite{crooks1999entropy, crooks2007measuring, feng2009far, sivak2012thermodynamic, habeck2017model}, including a result connecting the Jensen Shannon divergence.
%before drawing connections with hypothesis testing \cite{nielsen2013information, eguchi2006interpreting, coverthomas} in the Section \cref{sec:conjugate}.  

\subsection{Fluctuation Theorems in Physical Simulations}
Nonequilibrium fluctuations theorems \cite{crooks1999entropy} characterize the irreversibility of stochastic processes between thermodynamic states, and allow the estimation of equilibrium free energy differences from non-equilibrium simulations.  
Recalling the setting of \gls{AIS} in \cref{sec:ais}, we consider two equilibrium ensembles $\pi_0$ and $\pi_K$ with forward and reverse Markov transition kernels $\{ T_k(\vz_{k} |\vz_{k-1} ) \}_{k=1}^{K}$ and $\{ \tilde{T}_k (\vz_{k-1} |\vz_{k} ) \}_{k=1}^{K}$ governing transitions between states $\vz_k$ along time-dependent protocol parameterized by $\beta_k$.


Assuming that the Markov transitions obey detailed balance $T(\vz_{k}|\vz_{k-1}) \pi_{k}(\vz_{k-1}) = \tilde{T}(\vz_{k-1}|\vz_{k}) \pi_{k}(\vz_k)$ at each $k$, we can derive \gls{CFT} as: \footnote{The conditions for the \gls{CFT} are slightly more general than requiring detailed balance \cite{crooks1999entropy} and can be used with arbitrary energy functions \cite{habeck2017model}.  A common way of ensuring detailed balance is to use Metropolis Hastings accept/reject steps, which appear closely related to our likelihood ratio interpretation.}

\begin{align}
    \frac{P_f\chain}{P_r\revchain} &= \frac{\pi_0(\vz_0)}{\pi_K(\vz_K)} \prod \limits_{k=1}^K \frac{T_k(\vz_k|\vz_{k-1})}{\tilde{T}_k(\vz_{k-1}|\vz_{k})} = \frac{\pi_0(\vz_0)}{\pi_K(\vz_K)} \prod \limits_{k=1}^K \frac{\pi_k(\vz_k)}{\pi_k(\vz_{k-1})} \nonumber \\
    &= \frac{Z_K}{Z_0} \prod \limits_{k=1}^K \frac{f_{k-1}(\vz_k)}{f_k(\vz_k)} = \exp \{ W\chain - \Delta F \} \label{eq:pf_pr}
\end{align}
Physicists often associate a chain of forward $\chain$ or reverse $\revchain$ samples with a value of work, $W\chain = -\log w\chain = \sum_{k=0}^{K-1} (\beta_{k+1} - \beta_k) E(\vz_k)$, since this is quantity is measurable in physical simulation \cite{crooks1999entropy}.  The identity \eqref{eq:pf_pr} thus leads directly to the Jarzynski equality, as shown in Appendix \ref{app:fluctuations} or \citet{habeck2017model}.
%The distribution over chains $P_f\chain$ is  determined only by $W\chain$, and is then identical to the probability $p_f(W\chain)$ of observing a given value of work.  

Note that the work may simply be viewed as a sufficient statistic over \textit{chains} of samples, with each individual transition $T(\vz_{k}|\vz_{k-1})$ governed by the Hamiltonian  $ - \beta_k E(\vz) \}$.  This allows us to draw connections with the likelihood ratio exponential family in \cref{sec:path}, with  $-E(\vz) = \phi(\vz_k) = \log \frac{\pi_T}{\pi_0}.$

Let $\pi_0 = p_f(W)$ and $\pi_K = p_r(W) = p_f(W) \exp \{ -W + \Delta F \}$ be connected with a sequence of intermediate distributions parameterized by $\{ \beta_k \}_{k=1}^{K-1}$ or, more generally, a sequence of unnormalized Hamiltonians $f_k$.  Recall that the physical quantities include an extra negative sign compared with the probabilistic view, so that $\Delta F = \psi(\beta_0) - \psi(\beta_K)$ and 
\begin{align}
    - W = \log w &= - \sum_{k=0}^{K-1} (\beta_{k+1} - \beta_{k}) E(\vz_k | \vx) = \sum_{k=0}^{K-1} (\beta_{k+1} - \beta_{k}) \phi(\vz_k)  
\end{align}
We combine these expressions to draw parallels between the CFT and our path exponential family.  We write $W\chain$ to emphasize that the probability distributions are over sufficient statistics observed in sequences of samples $\vz_k \sim \pi_{\beta_k}$.
\begin{align}
    \pi_0 (W\chain) = p_f(W\chain) \quad \quad \pi_K = p_r(W\chain) &= p_f(W\chain) \exp \{ -W + \Delta F \} \label{eq:cft_exp_fam} \\
    &= p_f(W\chain) \exp \{ \sum_{k=0}^{K-1} (\beta_{k+1} - \beta_{k}) \phi_k(\vz_k) - \psi(\beta_K) \} 
\end{align}


%Given observations of forward and reverse processes, the Jarzynski equality $\langle \rangle$ suggests that we can estimate the free energy difference as the value of the work $W$ such that $p_f(W\chain) = p_r(W\revchain)$



% This setting of reversible \gls{MCMC} sampling chains is also known as bidirectional Monte Carlo \cite{grosse2015sandwiching, grosse2016measuring}.  \footnote{Note that more general or high dimensional conjugate variables may also be considered here.}  This section draws heavily upon \citet{habeck2017model}.

\subsection{Bennett's Acceptance Ratio }
\citet{shirts2003equilibrium} and \citet{crooks2007measuring} are both well written and explain these concepts in more detail.

Given a set of forward and reverse simulations, \gls{BAR} method \cite{bennett1976efficient} provides a maximum likelihood estimate of the free energy difference which would produce the given observations \cite{shirts2003equilibrium}.  The guiding intuition is to consider a classifier trained to predict whether the observed work arises from a forward ($\achain$) or reverse ($\arevchain$) sample chain or, in the single-sample case, from $\pi_0$ or $\pi_K$. We express these posterior probabilities as $P(f|W)$ and $P(r|W)$. 

%We will restrict our attention to the case of a single-sample chain for clarity, while the generalization follows

From the derivations above, we can interpret $P_f(W) = P(W|f) = \frac{P(W) P(f|W)}{P(f)}$.   With a prior defined by the proportion of simulations run in each direction $P(f) = \frac{n_f}{n_f + n_r} = 1- P(r)$, we can rewrite \eqref{eq:cft_fwd_rev} as
\begin{align*}
\exp \{ W - \Delta F \} &= \frac{P_f(W)}{P_r(W)} = \, \, \frac{\cancel{P(W)} P(f|W)}{P(f)} \frac{P(r)}{\cancel{P(W)} P(r|W)} \, \, = \, \, \frac{P(f|W)}{1-P(f|W)} \cdot \frac{1-P(f)}{P(f)} 
\end{align*}
Noting that $\frac{P(f)}{1-P(f)}= \frac{n_f}{n_r}$ and solving for $P(f|W)$
\begin{align}
    \frac{P(f|W)}{1-P(f|W)} &= \exp \{ W - \Delta F + \log \frac{n_f}{n_r} \} \quad \implies \quad P(f|W) = \frac{1}{1+\exp \{ -\big( W - \Delta F + \log \frac{n_f}{n_r} \big)\}} \label{eq:sigmoid_fwd} %\nonumber 
    %P(f|W) + \exp \{ W - \Delta F + R_f \} \, P(f|W) &= \exp \{ W - \Delta F + R_f \} \nonumber \\
\end{align}
Notice that this has the form of a sigmoid function, where the logit is based on the likelihood ratio $\frac{P_f(W)}{P_r(W)} = \exp \{ W - \Delta F \}$ times the `prior' sample proportion ratio $\frac{n_f}{n_r}$.  The posterior over the reverse chain can be similarly expressed, with the sign of the logit reversed $P(r|W) = (1+\exp \{ W - \Delta F + \log \frac{n_f}{n_r} \})^{-1}$.

Now we seek to maximize the log likelihood of the given sample chains being drawn according to the appropriate directions.  Note that this is a function of the free energy difference $\Delta F$, which informs the classifier \eqref{eq:sigmoid_fwd} at an observed work $W\chaini$ or $W\chainj$ and sample ratio $R_f$.
\begin{align}
    \log L(\Delta F) =  \sum \limits_{i=1}^{n_f} \underbrace{ \log (1+\exp \{ -\big( W - \Delta F + \log \frac{n_f}{n_r} \big) \})^{-1}}_{P(f|W)} +   \sum \limits_{j=1}^{n_r} \underbrace{ \log (1+\exp \{ W - \Delta F + \log \frac{n_f}{n_r} \})^{-1}}_{P(r|W)} \label{eq:bennett_lkd}
\end{align}
Differentiating the likelihood with respect to $\Delta F$ as in \cite{shirts2003equilibrium}, we see that
% \begin{align}
% \frac{d}{d \Delta F} \log L(\Delta F) &= \frac{d}{d \Delta F}   \sum \limits_{i=1}^{n_f} \log (1+\exp \{ - \big( W\chaini - \Delta F + R_f \big) \} )^{-1} \\ 
% &\phantom{=} + \frac{d}{d \Delta F}  \sum \limits_{j=1}^{n_r} \log (1+\exp \{ W\chainj - \Delta F + R_f  \})^{-1} \\
% &=  \sum \limits_{i=1}^{n_f} ( 1+ \exp \{ - \big( W\chaini - \Delta F + R_f \big) \}) \cdot \exp \{ - \big( W\chaini - \Delta F + R_f \big) \} \\
% &=\phantom{=} -  \sum \limits_{j=1}^{n_r} (1 + \exp \{ W\chainj - \Delta F + R_f  \}) \cdot \exp \{ W\chainj - \Delta F + R_f  \}
%  \end{align} 
% Each expression again corresponds to a sigmoid since $\sigma(x) = \frac{e^{x}}{1+e^{x}}=\frac{1}{1+e^{-x}}$.  However, now the forward samples are evaluated with respect to $P(r|W)$ and vice versa, thus measuring the probability of misclassification.  
the maximum likelihood free energy difference should yield equal total probability of error for the forward and reverse directions.  % then
%so that $\frac{d}{d \Delta F} \log L(\Delta F)$ implies 
\begin{align}
     \frac{d}{d \Delta F} \log L(\Delta F) = 0 \quad \implies \quad  \sum \limits_{i=1}^{n_f} P(r \, | \,W\chaini) \, = \,  \sum \limits_{j=1}^{n_r} P(f \, | \,W\chainj)
\end{align}
We will relate this to the Neyman-Pearson lemma later, in \cref{sec:neyman}.

Note that Bennett's Acceptance Ratio generalizes Annealed Importance Sampling, which considers only forward simulations, to various proportions of forward and reverse sample chains. 
   % &= \exp \{ -\big( W^{(i)} - \Delta F + R_f \big) \}  \sum \limits_{i=1}^{n_f} - &\exp \{ -\big( W^{(i)} - \Delta F + R_f \big) \}) + \exp \{  W^{(i)} - \Delta F + R_f \}  \sum \limits_{i=1}^{n_r} - \exp \{ W^{(i)} - \Delta F + R_f \}) \\
  % \sum \limits_{i=1}^{n_f} &\frac{\exp \{ -\big( W^{(i)} - \Delta F + R_f \big) \})}{ \sum \limits_{i=1}^{n_f}  \exp \{ \big( W^{(i)} - \Delta F + R_f \big) \}} =   \sum \limits_{i=1}^{n_r} \frac{\exp \{ W^{(i)} - \Delta F + R_f \})}{\sum \limits_{i=1}^{n_r} \exp \{ -\bigg( W^{(i)} - \Delta F + R_f \bigg) \}}

\subsection{Jensen Shannon Divergence}
\textcolor{red}{This is actually unsurprising as the JSD measures the mutual information between an indicator $I = \mathbb{I}(r(z) = \pi_0(z))$ and a sample drawn from a mixture $z \sim r(z) = ( 1- \lambda ) \pi_0 + \lambda \pi_1$. }
The log likelihood of the observed sample chains being drawn from the correct directional process simplifies as the sum of Jensen-Shannon divergences between adjacent state distributions \cite{crooks2007measuring} in the large sample limit.  Using our generalized Gibbs distribution with a base distribution $\pi_k(\vz) = \pi_0 \exp \{ - \beta_k E(\vz) - \psi(\beta_k) \} $ and letting $\lambda_f = \frac{n_f}{n_f + n_r}$, we derive the following expression for the \gls{BAR} likelihood \eqref{eq:bennett_lkd} in App. \ref{app:jensen}. 
% The derivations for the reverse direction follow similarly.
% \begin{align}
%   \sum \limits_{i=1}^{n_f} & \log (1+\exp \{ -\big( W\chaini - \Delta F + R_f \big) \} )^{-1} \\
%   &= -   \sum \limits_{i=1}^{n_f} \log \bigg( 1+\exp \big\{ - \bigg( \sum_{k=1}^K (\beta_{k} - \beta_{k-1}) E(\vz_k^{(i)}) - ( \psi(0) -\psi(\beta_K) ) + R_f \bigg) \big\} \bigg) \nonumber  \\ 
%   &= -   \sum \limits_{i=1}^{n_f} \log \bigg( 1+\exp \big\{ - \sum \limits_{k=1}^K \beta_{k} E(\vz_k^{(i)}) +  \sum \limits_{k=1}^K \beta_{k-1} E(\vz_k^{(i)})  + \sum \limits_{k=1}^{K} \big( \psi(\beta_{k-1})- \psi(\beta_k) \big) - R_f \big\} \bigg) \nonumber \\ 
%     &= -   \sum \limits_{i=1}^{n_f} \log \bigg( 1+\exp \big\{ \underbrace{- \sum \limits_{k=1}^K \beta_{k} E(\vz_k^{(i)}) - \sum \limits_{k=1}^{K}\psi(\beta_k) + \sum \limits_{k=1}^K \log \{ \pi_0 \} }_{\log \pi_{\beta_k}} - R_f \nonumber \\ 
%     & \phantom{-   \sum \limits_{i=1}^{n_f} \log \bigg( 1+\exp \{ \}  } \underbrace{+  \sum \limits_{k=1}^K \beta_{k-1} E(\vz_k^{(i)})  + \sum \limits_{k=1}^{K} \psi(\beta_{k-1})  - \sum \limits_{k=1}^K \log \{ \pi_0 \} }_{-\log \pi_{\beta_{k-1}}} \big\} \bigg) \nonumber \\ 
%     &= -  \sum \limits_{i=1}^{n_f} \log \bigg(  1 + \frac{\prod \limits_{k=1}^K  \pi_{\beta_{k}}(\vz_k^{(i)})}{\prod \limits_{k=1}^K  \pi_{\beta_{k-1}}(\vz_k^{(i)})} \frac{n_r}{n_f}   \bigg) \\
%     &= \phantom{-}  \sum \limits_{i=1}^{n_f} \log \frac{ n_f \cdot \prod \limits_{k=1}^K  \pi_{\beta_{k-1}}(\vz_k^{(i)}) }{ n_f \cdot \prod \limits_{k=1}^K  \pi_{\beta_{k-1}}(\vz_k^{(i)}) + n_r \cdot \prod \limits_{k=1}^K  \pi_{\beta_{k}}(\vz_k^{(i)}) }
% %   &= -  \sum \limits_{i=1}^{n_f} \log \bigg( 1+ \frac{\pi_{\beta_k}(\vz)} \cdot \frac{\ +  \sum \limits_{k=1}^K \beta_{k-1} E(\vz_k)  + \sum \limits_{k=1}^{K} \psi(\beta_{k-1}) - \sum \limits_{k=1}^{K}\psi(\beta_k)
% \end{align}
% where we have expanded the free energy difference into a telescoping sum $\psi(0) -\psi(\beta_K) = \sum_{k=1}^{K} \psi(\beta_{k-1}) -\psi(\beta_{k})$ and multiplied by $\pi_0 / \pi_0$.   Now, combining the forward and reverse sums, we obtain



% N_f , N_r VERSION
\begin{align}
    %  \log & L(\Delta F) =  \sum \limits_{i=1}^{n_f} \log (1+\exp \{ -\big( W\chaini - \Delta F + R_f \big) \} )^{-1} +  \sum \limits_{j=1}^{n_r} \log (1+\exp \{ W\chainj - \Delta F + R_f  \})^{-1} \nonumber \\
    %\phantom{L(\Delta F) }
     \log & L(\Delta F) \approx n_f \sum \limits_{k=1}^{K} D_{KL} [\pi_{\beta_{k-1}} || \frac{n_f}{n_f+n_r} \cdot \pi_{\beta_{k-1}} + \frac{n_r}{n_f+n_r} \cdot \pi_{\beta_{k}} ] + n_f K \log \frac{n_f}{n_f+n_r}  \label{eq:weighted_jsd} \\
     & \phantom{L(\Delta F) ===} + n_r \sum \limits_{k=1}^{K}  D_{KL} [\pi_{\beta_{k}} || \frac{n_f}{n_f+n_r} \cdot \pi_{\beta_{k-1}} + \frac{n_r}{n_f+n_r} \cdot \pi_{\beta_{k}} ] + n_r K \log \frac{n_r}{n_f+n_r} \nonumber  % +  \cdot n_r \cdot K \big( \log n_r + \log (n_f + n_r) \big)\\
\end{align}
where the approximation indicates the large sample limit when the empirical $n_f$ or $n_r$ observations approach the true expectation.  Note that this identity also holds for $K=1$, or a single sample chain and the task of distinguishing samples from $\pi_0$ and $\pi_1$.  For $n_f = n_r$, we recover a relationship with the \gls{JS} divergence.
\begin{align}
\log L(\Delta F)_{1/2} &=  n_f \sum \limits_{k=1}^{K} D_{KL} [\pi_{\beta_{k}} || \frac{\pi_{\beta_{k-1}} +  \pi_{\beta_{k}}}{2} ] +  D_{KL} [\pi_{\beta_{k-1}} || \frac{\pi_{\beta_{k-1}} + \pi_{\beta_{k}}}{2} ]  - 2 K \cdot n_f \log 2 \\ 
& = 2 n_f \cdot  \sum \limits_{k=1}^{K} D_{JS} [ \pi_{\beta_k}; \pi_{\beta_{k-1}} ] - K \cdot n_f \log 4
\end{align}
More generally, the expression in \eqref{eq:weighted_jsd} matches the `$\alpha$-skew Jensen-Shannon' divergence defined by \citet{nielsen2019generalization}, up to additive constant.  
Letting $\alpha = \frac{n_f}{n_f+n_r}$, the $\alpha$-skew \textsc{JSD} is asymmetric and can be written
\begin{align*}
    D_{JS}^{\alpha}[\pi_{\beta_{k-1}} ; \pi_{\beta_{k}}] = (1-\alpha) & D_{KL}[\pi_{\beta_{k-1}} || (1-\alpha)\pi_{\beta_{k-1}}  + \alpha \pi_{\beta_{k}}] \\
    \phantom{==} + \alpha \phantom{)} & D_{KL}[\pi_{\beta_{k}} \, \,  || (1-\alpha)\pi_{\beta_{k-1}}  + \alpha \pi_{\beta_{k}}]
    \end{align*}
These are $f$-divergences with generator $f_{\alpha}(x) = − \log  \big((1 - \alpha) + \alpha x \big) - x \log \big((1-\alpha) + \frac{\alpha}{x}}\big)$ and are bounded above by $H(\alpha)$ \cite{nielsen2019abstract}. %$\log \frac{1}{\alpha ( 1- \alpha)}$.
 
Finally, for $\alpha = 1/2$ or $n_f = n_r$, \citet{crooks2007measuring} show that the \gls{JS} divergence is related to two central geometric and thermodynamic quantities.  The Riemannian path length is also known as the thermodynamic length $\mathcal{L} = \int \limits_0^1 \sqrt{\frac{d\beta^i}{dt} g_{ij}(\beta(t)) \frac{d\beta_j}{dt} } dt $, where $g_{ij}$ indicates the Fisher information metric.    The integral of the Fisher information is referred to as the thermodynamic divergence $\mathcal{J} = \int \limits_0^1 \frac{d\beta^i}{dt} g_{ij}(\beta(t)) \frac{d\beta_j}{dt} dt$ and is proportional to the symmetrized KL divergence (\cite{bercher2012simple} Thm. 11, \cite{dabak2002relations} Eq. 14). The \gls{JS} divergence is then related as 
\begin{align}
    \mathcal{L} = \sqrt{8} \int d \sqrt{JS} \quad \quad \mathcal{J} = 8 \int d JS
\end{align*}
These results arise from the fact that the \gls{JS} divergence between infinitesimally close distributions can be written as \cite{crooks2007measuring, majtey2005wootters}.\textbf{verify} 
\begin{align*}
    JS(p; p+dp) = \frac{1}{8} \int \frac{1}{p(\vz)} \cdot \big( d p(\vz) \big)^2 d\vz
\end{align*}
%In the limit of $K \rightarrow \infty$ with $\beta_k$ infinitisemally close, the \gls{JS} divergence has differential:
%\begin{align}
%D_{JS}[\pi_{\beta};\pi_{\beta+d\beta}] = \frac{1}{8} \int d\pi_{\beta}(\vz)  d\log \pi_{\beta} (\vz) d\vz  %\textbf{Modify??}
%\end{align}


% This derivation has also been noted informally in \citet{stratos}.  The proof in \citet{mcallester2018formal}, which bounds the magnitude of mutual information which can be estimated with high confidence from $n$ samples as $I \leq \log n$, relies on similar ideas.


%Considering the transition between two adjacent states, say $\pi_{k-1}(\vz) \propto \pi_0(\vz) \exp \{ \beta_{k-1} E(\vz) \}$ and $\pi_k (\vz) \propto \pi_0(\vz) \exp \{ \beta_{k} E(\vz) \}$, we can simplify the log likelihood 


%When the posterior $\pi_K = \pzx$ is intractable, one might use an approximate sample which matches one of its modes \citet{habeck2017model} or use simulated data samples to produce a joint sample via $\pxz$. 


%In fact, BAR generalizes \gls{AIS}

%\subsubsection{Jensen Shannon Divergence}
\section{Hypothesis Testing}

%\section{Critical $\beta$ Values}\label{sec:conjugate}


Given a set of $n$ i.i.d. draws from a distribution $r(\vz)$, we consider a hypothesis test to distinguish between a null hypothesis $r = \pi_1$ or alternative hypothesis $r = \pi_0$.  The Neyman-Pearson lemma states that a likelihood ratio test forms the optimal decision rule for minimizing the type 1 error (false positive) rate subject to a given type 2 error (false positive) rate.  


% \subsubsection{Chernoff Information}
% The Chernoff information, which provides the optimal, asymptotic Bayes error exponent of a classifier distinguishing $\pi_0$ and $\pi_1$, is defined as 
% \begin{align*}
%     C(\pi_0, \pi_1) = - \min \limits_{0\leq \alpha \leq 1} \log \int \pi_0(\vz)^{1-\alpha} \pi_1(\vz)^{\alpha} \\
% \end{align*}
% This can be derived by noting that $P_e = \int \min (\pi_0(\vz), \pi_1(\vz)) d\vz \leq \min \int \pi_0^{1-\alpha} \pi_1^{\alpha}$.  A more satisfying derivation may also be given using Sanov's Thm (\citet{coverthomas} Ch. 11.8).

% Note that, by taking the asymptotic limit, this formulation washes out the effect of prior probabilities over the sampling distribution, i.e. $\lambda_0 = \frac{n_f}{n_f + n_r}$ and  $\lambda_1 = 1-\lambda_0 = \frac{n_r}{n_f + n_r}$ in analogy with the forward/reverse transitions above, with $P_{err} = \lambda_0 P_{err}(\pi_1| \pi_0) + (1- \lambda_0) P_{err}(\pi_0| \pi_1) $.
    
% The quantity to be minimized clearly corresponds to the log partition function in our path exponential family. We can write this point in a number of different ways (see below), but note that, at $\alpha^{*}$
% \begin{align*}
%     D_{KL}[\pi_{\alpha^{*}} || \pi_0] =D_{KL}[\pi_{\alpha^{*}} || \pi_1]
% \end{align*}
% The optimal decision rule is a likelihood ratio test (by Neyman-Pearson lemma) using MAP rule
% \begin{align}
%     \text{Accept hypothesis $r = \pi_0$ if : } \frac{\phantom{(1-} \lambda_0\phantom{)} \prod \limits_{i=1}^{n} \pi_0(z^{(i)} |x) }{(1-\lambda_0) \prod \limits_{i=1}^{n} \pi_1(z^{(i)} |x)} > 1 \quad \text{(and vice versa)} \label{eq:map_decision}
% \end{align}


 \paragraph{Conjugate Function:}
% It is interesting to consider $\eta = 0$ so that $\eta = \mathbb{E}_{\pi_{\beta}} \log \pxgz - \log \px = 0$ as in \eqref{eq:eta}.  This simply implies $\mathbb{E}_{\pi_{\beta}} \log \pxgz = \log \px$.  The conjugate optimization $\psi^{*}(0)$ then becomes
% \begin{align}
% \psi^{*}_z(0) = \sup \limits_{\beta^{\prime}}  \beta^{\prime} \cdot 0 - \psi(\beta^{\prime}) = \inf \limits_{\beta^{\prime}} \psi(\beta^{\prime})
% \end{align}
% This is equivalent to the optimization in \eqref{eq:choosing_renyi}, so that our optimal $\alpha$ corresponds to the point where $\mathbb{E}_{\pi_{\beta}} \log \pxgz = \log \px$.  
For the path exponential family with base distribution $\pi_0$, the conjugate takes the form of a KL divergence.
\begin{align}
\psi^{*}(\eta_{\beta}) = D_{KL}[\pi_{\beta}(\vz|\vx) || \pi_0(\vz|\vx)]
\end{align}

\subsection{Ways of Writing the Chernoff Information point $\alpha^{*}$}
 The Chernoff information \citet{nielsen2011chernoff,nielsen2013information}, and corresponding Renyi divergence of order $\alpha^{*}$,  provides the tightest upper bound on the Bayes error of a hypothesis test distinguishing samples from $\pi_0$ and $\pi_1$.


\begin{itemize}[leftmargin=*]
\item Maximum Jensen Gap w/ $\beta_0 = 0$, $\beta_1 = 1$, mixing measure $\alpha$ (holds for any $\{\beta_k\}_{k=0}^K$, $K$) \cite{Banerjee2005}
    \begin{align*}
        \mathcal{J}_{\alpha, \psi} &= (1-\alpha) D_{KL}[\pi_{\alpha} || \pi_0 ]+ \alpha D_{KL}[\pi_{\alpha} || \pi_1] \\
        &= (1-\alpha) \psi(0) + \alpha \psi(1) - \psi(\alpha) \\
        &= (1-\alpha) D_{\alpha}[\pi_1 || \pi_0] \\
        &= - \psi(\alpha) \quad \text{\small (when $\psi(0) = \psi(1) = 0$)}
    \end{align*}
\item Renyi Divergence as a Jensen's gap (2nd to last line) shown in \cite{nielsen2011renyi}, App. \ref{app:renyi}
\item $(1-\alpha) D_{\alpha}[\pi_1 || \pi_0]$ concave \cite{van2014renyi}, also equals $-\psi(\beta)=-\psi(\alpha^{*})$ of (convex) R-D exp family partition
      \begin{align*}
    \max \limits_{\alpha} \mathcal{J}_{\alpha, \psi} &= \max \limits_{\alpha} (1-\alpha) D_{\alpha}[\pi_1 || \pi_0] = \min \limits_{\alpha} \psi(\alpha) = -\psi(\alpha^{*})
     \end{align*}
\item At this point, note that the gradient of $\mathcal{J}_{\alpha, \psi}$ with respect to $\alpha$ is 0, i.e. $\frac{d}{d\alpha} (1-\alpha) D_{KL}[\pi_{\alpha} || \pi_0 ]+ \alpha D_{KL}[\pi_{\alpha} || \pi_1] = 0$.  This implies that the two quantities in this additive mixture are equal at $\alpha^{*}$.
\begin{align*}
    D_{KL}[\pi_{\alpha^{*}} || \pi_0 ] = D_{KL}[\pi_{\alpha^{*}} || \pi_1]
\end{align*}
\end{itemize}

\end{itemize}

% \begin{figure*}[t]
% \includegraphics[width=.95\textwidth]{figs/alpha_star.pdf}
% \end{figure*}

We can see directly that $(\alpha-1) D_{\alpha}[\pzx||\qzx] = \psi(\alpha)$ from the definition of the Renyi divergence.
\begin{align}
D_{\alpha}[\pzx||\qzx] = \frac{1}{\alpha-1} \log \int \qzx^{1-\alpha} \pzx^{\alpha} d\vz 
\end{align}
Thus, we have $\psi(\alpha) = (\alpha - 1) D_{\alpha}[\pzx||\qzx]$.   \citet{van2014renyi} demonstrate that the function $(1-\alpha) D_{\alpha}$ is concave in $\alpha$, indicating that we can find its maximum or the corresponding minimum of $\psi$. 
\begin{align}
\max \limits_{\alpha} (1-\alpha) D_{\alpha}[\pzx||\qzx] &= \min \limits_{\alpha} \psi(\alpha) \label{eq:choosing_renyi}
\end{align}




%\paragraph{Chernoff Information:}  Imagine a hypothesis test to distinguish samples from two distributions $\qzx$ and $\pzx$, with 

% Furthermore, this minimum and corresponding order of the Renyi divergence correspond the Chernoff information \citet{nielsen2011chernoff,nielsen2013information}, which provides the tightest upper bound on the Bayes error of a hypothesis test distinguishing samples from $\pzx$ and $\qzx$.



% \subsection{Neyman-Pearson Lemma and Sanov's Theorem: }\label{sec:neyman} 
% \citet{eguchi2006interpreting}, \citet{coverthomas} 11.7 and 11.9

% Consider a likelihood ratio test from samples $z_{1:N}$ to distinguish the hypotheses $z_{1:N} \sim \pi_0$ or $z_{1:N} \sim \pi_1$ (drawn iid in both cases).  The proof is given by the method of types, assuming discrete support $\mathcal{Z}$ so that the probability is determined only by the empirical counts of $\delta(z_i, \mathpzc{z} )$ for each $\mathpzc{z} \in \mathcal{Z}$ and observed $z_i$ \footnote{For example, the type of a binary sequence $01001$ would be $(3, 2)$ over the support $(z=0, z=1)$}.  Denote this distribution $P_{Z_n}(\mathpzc{z})$.  Note that we can also evaluate $\pi_0(\mathpzc{z})$, e.g., if the supports overlap.

% Similar reasonsing should hold in the general case as well (\textbf{working on generalizing to continuous support}).  
% %Writing the implicit density induced by this procedure (for example, with priors of $p(z_{1:N} \sim \pi_0) = \lambda$ and $p(z_{1:N} \sim \pi_1) = 1-\lambda$)).
% \begin{align*}
%     L(z_{1:N}) &= \log \frac{\pi_0(z_{1:N} ) }{\pi_1(z_{1:N} ) } \\
%     &= \sum_{i=1}^{N} \log \frac{\pi_0(z_{i} ) }{\pi_1(z_{i} ) } \\
%     &= \sum_{\mathpzc{z} \in \mathcal{Z}} n \cdot P_{Z_n}(\mathpzc{z}) \log  \frac{\pi_0(\mathpzc{z} ) }{\pi_1(\mathpzc{z} ) } \frac{ P_{Z_n}(\mathpzc{z})}{ P_{Z_n}(\mathpzc{z})} \\
%     &= n D_{KL} [ P_{Z_n}(\mathpzc{z}) || \pi_1] - n  D_{KL} [ P_{Z_n}(\mathpzc{z}) || \pi_0]
% \end{align*}
% We often choose a threshold for the likelihood ratio test, so that if $\exp \{ L(z_{1:N}) \} \geq T$, then we accept the hypothesis $z_{1:N} \sim \pi_0$.  Thus, the likelihood ratio decision rule, which is optimal  by  the Neyman-Pearson lemma, corresponds to a KL divergence comparison:
% \begin{align*}
%     n D_{KL} [ P_{Z_n}(\mathpzc{z}) || \pi_1] - n  D_{KL} [ P_{Z_n}(\mathpzc{z}) || \pi_0] \geq \log T
% \end{align*}
% We will make analogy with the Chernoff information point, so that $P_{Z_n}(\mathpzc{z}) = \pi_{\alpha}(z|x)$.  At  $ \pi_{\alpha^{*}}(z|x)$, we have $D_{KL}[\pi_{\alpha^{*}}||\pi_{0} ] = D_{KL}[\pi_{\alpha^{*}}||\pi_{1} ]$, implying a decision threshold of $\log T = 0 \implies T = 1$.  Thus, we accept $z_{1:N} \sim \pi_0$ only if it has higher likelihood of generating the samples.  This is in exact correspondence with the asymptotically optimal MAP decision rule in \eqref{eq:map_decision}


% \paragraph{Sanov's Theorem: } \cite{coverthomas} Ch. 11, related to Pythagorean Theorem and mismatched decoding in \citet{latham2005synergy}

% We will make an error if draws from $\pi_1$ appear to have higher likelihood than actual draws from $\pi_0$, fooling the likelihood ratio test.  The probability of this event is treated by large deviation theory.    

% Namely, for the convex set defined by (empirical) expectation constraints $\frac{1}{n}\sum \phi(\vz_i) = \eta$, the asymptotic probability of draws from $\pi_0$ appearing in this set is given by the minimum KL divergence to this set.  This minimizer is given by the path exponential family with base distribution $\pi_0$ and sufficient statistics $\phi(\vz_i)$.
% \begin{align*}
%     \lim \limits_{n\rightarrow \infty \frac{1}{n} \log Pr( \frac{1}{n} \phi(\vz) \in \Pi ) = - \min D_{KL}[ \mathcal{M} || \pi_0] = - D_{KL}[\frac{\pi_0 \exp \{ \alpha \phi(\vz) \} }{Z_{\alpha}} || \pi_0 ]
% \end{align*}





% \subsubsection{Conjugate Function}  
% Since the partition function $\psi(\beta)$ is convex, we can consider its conjugate dual $\psi^{*}(\eta)$ as a function of the mean parameter $\eta = \nabla \psi(\beta)$.  
% \begin{align}
% \psi^{*}(\eta) &= \sup \limits_{\beta^{\prime}} \beta^{\prime} \cdot \eta - \psi(\beta^{\prime}) \label{eq:conj} =  \beta_{\eta} \cdot \eta - \psi(\beta_{\eta})
% \end{align}
% where, by differentiating wrt $\beta$, one can verify that the $\sup$ is attained when $ \eta = \nabla_{\beta} \psi(\beta^{\prime})$.   Thus, for a given argument $\eta$, the conjugate optimization corresponds to the Legendre transform, finding $\beta_{\eta}$ such that $ \eta_{\beta} = \nabla_{\beta} \psi(\beta_{\eta}) = \mathbb{E}_{\pi_{\beta_{\eta}}}[T(\vx,\vz)]$.  









% \subsection{Jensen Gaps vs. Jensen Shannon Divergence}
% It is also interesting to note that, since the KL divergence is jointly convex in the pair, $(p_0, p_1), (q_0, q_1)$, we can apply Jensen's inequality on each Bregman information $\mathbb{E}_{\nu}\big [D_{f}[p_i || \mathbb{E}_{\nu}[p_i]\big]$.   Note that these inequalities are valid for distributions outside our exponential family as well, and we use $r$ to indicate an arbitrary distribution which is optimized over in \eqref{eq:jg_min_primal} or \eqref{eq:jg_min_dual}. 
% \begin{align}
% D_{KL}[ \, r \, || (1-\alpha) \pi_0 + \alpha \pi_1] \leq (1-\alpha) D_{KL}[ \, r || \pi_0] + \alpha D_{KL}[ \, r || \pi_1] \label{eq:jsd_jg_ineq_primal}
% \end{align}
% Note that the left hand side is equal to the (skew) Jensen-Shannon divergence \eqref{eq:weighted_jsd}.  On the right side, we obtain the mixture of KL divergences which is minimized by $\mathcal{J}_{\alpha, \psi}$ in \eqref{eq:jg_primal}, with 
% \begin{align}
%     r^{*} &= \argmin_{r}  (1-\alpha) D_{KL}[ \, r || \pi_0] + \alpha D_{KL}[ \, r || \pi_1] = \frac{\pi_0^{1-\alpha} \pi_1^{\alpha}}{Z_{\alpha}} \\
%     \implies D_{KL}[ \, \pi_{\alpha} \, || (1-\alpha) \pi_0 + \alpha \pi_1] \leq 
% \end{align}
% This may be verified by variational calculus without relying on exponential families, and is also described in \cite{grosse2013annealing}.   The inequality in \eqref{eq:jsd_jg_ineq_primal} is tight if and only if $\pi_0 = \pi_1$.  
% In the reverse direction, corresponding to $D_{\psi^{*}}$ and $\mathcal{J}_{\lambda, \psi^{*}}$, we obtain
% \begin{align*}
%     D_{KL}[  \lambda \pi_0 + (1-\lambda) \pi_1 || r ] \leq \lambda D_{KL}[ \pi_0 || r ] + (1-\lambda) D_{KL}[ \pi_1 || r ] \label{eq:jsd_jg_ineq_dual}
% \end{align*}
%   \begin{align}
%       r^{*} &= \argmin_{r}  (1-\alpha) D_{KL}[ \, r || \pi_0] + \alpha D_{KL}[ \, r || \pi_1] \\
%     &= \frac{\pi_0^{1-\alpha} \pi_1^{\alpha}}{Z_{\alpha}}
%   \end{align} 



% \clearpage
% \section{Information Geometric Projections}
% \begin{figure*}[h]
% \begin{minipage}{.45\textwidth}
% \includegraphics[width=.99\textwidth]{figs/e_bisector.pdf}
% \captionof{figure}{The bisector hyperplane $r$ s.t. $D_{KL}[r(\vz|\vx)||\pi_0] = D_{KL}[r(\vz|\vx)||\pi_1] $ is orthogonal to the geometric mixture curve connecting $\pi_0$ and $\pi_1$ (\citet{nielsen2007bregman}). }\label{fig:e_bisector}
% \end{minipage}\hspace{.5cm}
% \begin{minipage}{.45\textwidth}
% \includegraphics[width=.99\textwidth]{figs/rd_proj.pdf}
% \captionof{figure}{The $e$-projection of $\qz$ onto the manifold defined by expectation constraints $r(\vz|\vx)$ s.t. $\mathbb{E}_r \log \pxgz = D$ is defined as the orthogonal intersection point where $\mathbb{E}_{\pi_{\beta}} \log \pxgz = D$ where $\pi_{\beta} = \qz \exp^{\beta \log \pxgz } / \Psi(\beta)$ as in Sec. \ref{sec:path}.}\label{fig:rd_proj}
% \end{minipage}
% \end{figure*}

% \subsection{Bisector is Orthogonal at $\alpha^{*}$}

% \subsection{Rate-Distortion and the $e$-Projection of $\qz$ onto Expected Sufficient Statistics Manifold}
% %e -project marginal q(z) onto manifold of expectation constraints q(z|x) via p(z|x) geodesic

% \subsection{Maximum Likelihood and the $m$-Projection of Data $\qx$ onto Model Params} 
% \citet{amari2016information} 2.8.3
%m -project data(x) onto manifold of model



% Sanov's theorem for continuous variables  \cite{csiszar2006simple}




% \section{Annealed Rate-Distortion}
% \paragraph{Jensen's Gap:}
% \paragraph{Pythagorean Theorem:} 
% \paragraph{Bercher Construction:} 
% \paragraph{E Step: $\min D_{KL}[\qzx || \qz \pxgz^{\beta} / Z_{\beta}]$} 

==> sections/app/q.tex <==
\section{Q-Gaussians}
\begin{align*}
    p_{q, \gamma}(\omega) = \frac{r_0(\omega)}{Z(\gamma, m)} [ 1 + \gamma (\omega - m)]_{+}^{-\frac{1}{q}-1} = \frac{r_0(\omega)}{Z(\gamma, m)} [ 1 - \gamma (\omega - m)]_{+}^{\frac{q}{1-q}}\label{eq: q_gaussian}
\end{align*}
where the domain $\omega \in \Omega$ is restricted to $\omega \geq m$. \textcolor{red}{ which is also indicated with the notation $[x]_{+} = \max \{ x, 0 \} $ }.

Tsallis introduced the $q$-Gaussian in the context of \textit{nonextensive thermodynamics}, where it achieves remarkable correspondence with experimental observations.  The $q$-Gaussian is also related to the generalized Pareto distribution, which has been used to regularize and diagnose heavy tails in importance sampling \cite{vehtari2015pareto,yao2018yes} \footnote{Our notation in \eqref{eq:q_gaussian} is perhaps non-standard in order to align with the parameter $k$ in this literature \cite{vehtari2015pareto,yao2018yes}.}
Indeed, the $q$-Gaussian arises from seeking the maximum entropy `tail distribution' $P_t(\omega ; m) = P(\omega | \omega \geq m)$ subject to a constraint on $D_{KL}[P_t || P]$, which sets the order $q$, and the standard moment constraint, which sets the scale $\gamma$ \cite{bercher2008tsallis}.

\subsection{$q$-Exponential Family}
The $q$-Gaussian may be derived as an exponential family using a generalized exponent $\exp_q$, for which we can also define a logarithm $\log_q$
\begin{align*}
    \exp_q (u) &= \big[1 + (1-q) u \big]^{\frac{1}{1-q}} \quad \quad \quad \log_q (u) = \frac{1}{1-q} \big( u^{1-q} - 1 \big)
\end{align*}
As $q \rightarrow 1$, we recover the traditional $\exp$ and $\log$.   Similarly to the traditional case, we can construct exponential families of distributions based on parameters $\theta$, sufficient statistics $\phi(\omega)$, and base measure $\pi_0(\omega)$.
\begin{align*}
r_{q, \theta} (\omega) &= \pi_0(\omega) \, \exp_q \{ \theta \cdot \phi(\omega) - \psi_{q} (\theta) \} \\
&= \pi_0(\omega) \big[ 1+ (1-q)\cdot \big( \theta \cdot \phi(\omega) - \psi_{q} (\theta) \big) \big]^{\frac{1}{1-q}}
\end{align*}
\textcolor{red}{substitute $\psi_{q} (\theta) \approx \theta \cdot \eta_q - \psi^{*}_{q} (\theta) $}... still normalized? 

The normalizing constant $\psi_{q} (\theta)$ is such that
\begin{align*}
    \int_{\Omega} \pi_0(\omega) \big[ 1+ (1-q)\cdot \big( \theta \cdot \phi(\omega) - \psi_{q} (\theta) \big) \big]^{\frac{1}{1-q}} = 1
\end{align*}
As shown in \cref{app:conv}, the $q$-free energy is convex with the following first and second derivatives.
\begin{align*}
    \eta_q := \frac{\partial \psi_q}{\partial \theta } = \int \frac{\pi_0(\omega)^{1-q} r_{q, \theta} (\omega)^{q}}{\int \pi_0(\omega)^{1-q} r_{q, \theta} (\omega)^{q} d \omega } \phi(\omega) d\omega =  \frac{1}{Z(q, \theta)} \int \pi_0(\omega) \big[ 1+ (1-q)\cdot \big( \theta \cdot \phi(\omega) - \psi_{q} (\theta) \big) \big]^{\frac{q}{1-q}} \cdot \phi(\omega) d\omega  \\
\end{align*}
\textcolor{red}{Note, $\frac{\partial \pi_{\beta}}{\partial \beta} = \pi_{\beta} \cdot (\phi(\omega) - \eta_{\beta})$ could be shown}.

The $q$-Gaussian appears as a special case of the $q$-exponential family with 

The conjugate dual function for the $q$-free energy (with no base distribution) can be written as
\begin{align*}
    \psi^{*}_q(\eta) &= \theta_{\eta} \cdot \eta - \psi_q(\theta_{\eta}) \\
    &= \frac{1}{1-q} \big( \frac{1}{\int \pi_0(\omega)^{1-q} r_{q, \theta} (\omega)^{q} } -1 \big)
\end{align*}
\textcolor{red}{However, the non-additivity of $\log_q$ means it is difficult to translate this expression }




==> sections/main/hypothesis_testing.tex <==

\section{Hypothesis Testing}
In this section, interpret the likelihood ratio exponential family as being intimately related to hypothesis testing as to whether samples were drawn from a base distribution $\pi_0(\vz)$ or target $\pi_1(\vz)$.  
%While we present these connections in general terms, the examples of the previous section correspond to the prior or approximate posterior as $\pi_0(\vz)$, and the target $\pi_1(\vz)$ as the posterior over latent variables given the data point $\vx$, model parameters $\theta$, and possibly the label $y(\vx)$.


\subsection{Sanov's Theorem: } \label{sec:sanov} 
% It is well known that exponential family of distributions arises from maximizing entropy or minimizing a KL divergence subject to a expectation constraint $\mathbb{E}[\phi(z)] = \eta$.  The optimizing distribution \eqref{eq:path_exp_family_general} is also known as the $e$-projection \cite{amari2016information} or $I$-projection \cite{csiszar2004information}.
An alternative view of the exponential family is given by Sanov's Theorem and large deviation theory ( \cite{cover2012elements} Ch. 11, \cite{csiszar1984sanov,csiszar2004information}).  Let $M_{\pi_0, \eta}$ denote the event that i.i.d. draws $\{ z_i \}_{i=1}^{N}$ from a distribution $\pi_0(z)$ will yield the set of empirical expectations given by $\mybar{\eta} = \{\mybar{\eta_j} = \frac{1}{N} \sum_i \phi_j(z_i)\}_{j=1}^{M}$. 
\begin{align}
\hspace*{-.2cm}	\lim \limits_{n \rightarrow \infty} \frac{1}{n} Pr(M_{\pi_0, \mybar{\eta}}) \rightarrow \exp \{ -\kl[r^{*}(\z) || \pi_0(\z) ] \}  \, \, \text{ where } r^{*}(z) = \min \limits_{r \in \mathcal{M}_{\mybar{\eta}}} \kl[r(\z)|| \pi_0(\z)] \label{eq:sanov0}
\end{align}
The probability of observed the desired expectation constaints $\mybar{\eta}$ is thus determined by $r^{*}(z)$, the `closest' distribution to $\pi_0$ within the feasible set \cite{eguchi2006interpreting, cover2012elements}.   This solution $r^{*}$ will correspond with a distribution $\pi_{\beta_{\mybar{\eta}}}$ and the supremum of the conjugate optimization \eqref{eq:conjugate}-\eqref{eq:legendre_sol}.
% This is simply the definition of the $e-$projection when the divergence is measured using $\kl[r || \pi_0]$.

% Projection is defined according to an affine connection $\nabla$ and a metric tensor $g$.
% When the space is dually flat it amounts to minimize a Bregman divergence which is realized by the KL divergence for the manifold of an exponential family.


\subsection{Neyman Pearson Lemma: } \label{sec:neyman_pearson}

Suppose we have access to $n$ i.i.d. observations from an unknown distribution $r(z)$, and are interested in testing the hypotheses that either $H_0: r(z) = \pi_0(\z)$ or $H_1: r(z) = \pi_1(\z)$.  The Neyman-Pearson lemma states that the likelihood ratio test with threshold $\eta$ is optimal, in the sense that, for any other decision region with type-1 error $Pr(e_1) = R$, then the type-2 error for this region is greater than or equal to that of the likelihood ratio test  \footnote{Let this usage of $\eta$ refer to the case of a single sufficient statistic $\phi(z) = \log \frac{\pi_1}{\pi_0}$} \cite{coverthomas, borade2006projection}.    The decision rule is given by
\begin{align}
A_{n}(\pi_1; \bar{\eta})  = \bigg \{ \, z_{1:n} \, \, \bigg | \, \, \, \frac{1}{n} \sum \limits_{i=1}^n \log \frac{\pi_1(z_i)}{\pi_0(z_i)} \geq \bar{\eta}  \, \bigg \}
\end{align}

In the previous section, we found that Sanov's theorem yields the probability of an event $M_{\pi_0, \eta}$, that draws from $\pi_0$ obtain an empirical likelihood ratio $\frac{1}{N} \sum_i \phi(z_i) = \frac{1}{N} \sum_i \log \frac{\pi_1}{\pi_0} \geq \eta$.   This simply corresponds to the probability of error in accepting $r(z) = \pi_1$ when the observations were truly drawn from $\pi_0$ and is governed by $D_{KL}[\pi_{\beta}(z) || \pi_0]$.

We may also consider the other type of error, in which draws from $\pi_1$ attain an average likelihood ratio $\frac{1}{N} \sum_i \log \frac{\pi_1}{\pi_0} \leq \eta$ and the hypothesis $r(z) = \pi_0(z)$ is accepted.  The error probability is similarly given by Sanov's theorem %by the $e-$projection of $\pi_1$ onto the manifold $\mathcal{M}_{\eta}$.
\begin{align}
r^{*}(z) &= \argmin \limits_{r \in \mathcal{M}_{\eta}} D_{KL}[r(z) || \pi_1] = \frac{1}{Z_{\beta^{\prime}}} \, \pi_1(z) \exp \{ \beta^{\prime} \cdot \log \frac{\pi_1(z)}{\pi_0(z)} \} \propto \pi_0(z)^{-\beta^{\prime}} \cdot \pi_1(z)^{1+\beta^{\prime}} \label{eq:sanov1}
\end{align}
By simply reparameterizing the Lagrange multiplier $\beta^{\prime} = \beta_t -1$, we can see that this solution for  $\pi_1$ matches that for $\pi_0$ and corresponds to a distribution in the likelihood ratio exponential family.   In \cref{fig:sanov}, we visualize the geometric mixture path connecting $\pi_0$ and $\pi_1$ intersecting the feasible set $\mathcal{M}_{\eta}$, which occurs with a right angle due to a generalization of the Pythagorean Theorem to the KL divergence (\cite{nielsen2018information}, \cite{amari2016information} Sec. 1.6 and 2.8).


Thus, the likelihood ratio test provides the optimal decision rule for hypothesis testing, with the asymptotic error probabilities governed by $D_{KL}[\pi_{\beta_t}(z) || \pi_0(z)]$ and $D_{KL}[\pi_{\beta_t}(z) || \pi_1(z)]$. Sanov's theorem and Eqs. \eqref{eq:sanov0} and \eqref{eq:sanov1} thereby allow us to express the Neyman Pearson lemma using KL divergences.  For a given type 1 error $R$, we see that $r^{*}$ is the solution to the following optimization
\begin{align*}
r^{*}(z) = \argmin D_{KL}[\pi_{\beta_t}(z) || \pi_1(z)] \quad \text{subj. to } D_{KL}[\pi_{\beta_t}(z) || \pi_0(z)] = R
\end{align*}
Introducing a Lagrange multiplier to enforce the constraint, we can write this optimzation as 
\begin{align}
     \argmin D_{KL}[\pi_{\beta_t}(z) || \pi_1(z)] - \lambda \big(  D_{KL}[\pi_{\beta_t}(z) || \pi_0(z)] -  R \big) \label{eq:lagr_np}
\end{align}
Parameterizing the Lagrange multiplier as $\lambda = \frac{t}{1-t}$, which has a domain of $\lambda \in [0, \infty)$ for $t \in [0,1]$, we see that the optimization \eqref{eq:lagr_np} matches the variational representation \eqref{eq:vrep1}, up to a factor of $\frac{1}{1-t}$ and additive constant $R$.   

Note that likelihood ratio threshold $\mybar{\eta}$ corresponds to the error region threshold $R = \psi^{*}(\mybar{eta}) = D_{KL}[\pi_{\beta_t} || \pi_0]$ where $\beta_t = \beta_{\mybar{\eta}}$ for some mixing parameter $t$.   Thus, we conclude from \eqref{eq:lkd_ratio_fam}, \eqref{eq:vrep1}, and \eqref{eq:lagr_np} that any intermediate distribution $\beta_t$ in the likelihood ratio exponential family corresponds to a decision region size and threshold in the Neyman-Pearson lemma.

\subsection{Chernoff Information}
While each choice of $\beta_{t}$ determines a likelihood ratio test and error region, how should we choose this parameter?   Regardless of the prior probabilities $p_0, p_1$ which we might assign to each hypothesis in a Bayesian setting, the Chernoff information provides the best achievable error exponent in the large sample limit \cite{nielsen2013information,coverthomas}.
\begin{align}
C^{*} = - \min \limits_{\beta} \, \log \int \pi_0(z)^{1-\beta} \pi_1(z)^{\beta} dz
\end{align}
At this optimum, we show in \cref{app:equal_kl} that 
\begin{align}
D_{KL}[\pi_{\beta}(z) || \pi_0(z)] = D_{KL}[\pi_{\beta}(z) || \pi_1(z)]
\end{align}
and the optimal decision rule is given by a threshold of $\eta_{\beta} = \mathbb{E}_{\pi_{\beta}} \log \frac{\pi_1(\z)}{\pi_0(\z)} = 0 $.  


\begin{figure*}[t]
\begin{minipage}{.35\textwidth}
%\begin{subfigure}{.475\textwidth}
\includegraphics[width=.9\textwidth]{figs/sanov.pdf}
\caption{Sanov's Theorem and the Likelihood Ratio Test} \label{fig:sanov} 
%:  For a given acceptance threshold $\bar{\eta}$, which defines an optimal tradeoff between size of the type 1 and type 2 error regions in the Neyman-Pearson lemma, we can define a manifold of distributions $\mathcal{M}_{\bar{\eta}}$ satisfying $\mathbb{E}_r[\log \pi_1 / \pi_0] = \bar{\eta}$.   Using Sanov's Theorem, we can see that the minimizers of both $D_{KL}[r \, ||\pi_1]$ and $D_{KL}[r \, ||\pi_0]$ for $r \in \mathcal{M}_{\bar{\eta}}$ will coincide, with $r^{*}(\vz|\vx) = \pi_{\beta}(\vz|\vx) \propto \pi_0^{1-\beta} \, \pi_1^{\beta}$ for $\beta$ such that $\eta_{\beta} = \mathbb{E}_{\pi_{\beta}}[\phi] = \bar{\eta}$.
\end{minipage}\hspace{.1cm}
\begin{minipage}{.65\textwidth}
\includegraphics[width=\textwidth]{figs/alpha_star.pdf}
\caption{Chernoff Information of the graphs of $\psi(\beta)$ and $\eta_{\beta} = \frac{d}{d\beta}\psi(\beta)$.} \label{fig:chernoff} 
\end{minipage}
\end{figure*}


==> sections/main/intro.tex <==
\section{Introduction}
%%%%%%%

The exponential families, or Gibbs distributions, are well known in machine learning and statistical physics as the maximum entropy distributions subject to a set of observed constraints \cite{jaynes1957information} and encompass many familiar parametric distributions \cite{nielsen2009statistical}.  In this paper, we present \textit{likelihood ratio} exponential families, which can be constructed between arbitrary distributions that are not in an exponential family themselves.  A sequence of intermediate distributions in our family also matches the geometric mixture path found in methods as \gls{AIS} \cite{jarzynski1997equilibrium, neal2001annealed}.  

We provide additional perspective on this  exponential family in terms of hypothesis testing and the Neyman-Pearson lemma, which states that the likelihood ratio test is the optimal decision rule for inferring whether observed samples were drawn from a base distribution or a target distribution.   In particular, any intermediate distribution in our family may be given a variational representation minimizing a mixture of $\textsc{kl}$ divergences \cite{grosse2013annealing}, which also corresponds to the asymptotic trade-off between type-1 and type-2 error at a given threshold.   The critical point of this tradeoff corresponds to the Chernoff information (\cite{cover2012elements} Ch.11, \cite{nielsen2013information}), which we proceed to discuss in the context of marginal likelihood estimation in generative models.

While a particular likelihood ratio family was used to analyse the recent \gls{TVO} \cite{masrani2019thermodynamic} in \cite{brekelmans2020all}, we provide a more general analysis which includes \gls{RD} optimization (\cite{cover2012elements} Ch. 10, \cite{alemi2018fixing, huang2020augmented}) and extensions with sufficient statistics for classification or generalization \cite{alemi2018therml, gao2020free} as in the \gls{IB} \cite{tishby1999information} method.   Leveraging our exponential family perspective, we interpret these methods in terms of Legendre duality \cite{amari2016information, wainwrightjordan}.

% In this paper, we present likelihood ratio exponential families, which have log importance weights as their sufficient statistics and can be constructed between arbitrary distributions.  This construction matches the geometric mixture path found in \gls{AIS} \cite{jarzynski1997equilibrium, neal2001annealed}, the \gls{TVO} \cite{masrani2019thermodynamic, brekelmans2020all},  \gls{RD} optimization (\cite{cover2012elements} Ch. 10, \cite{alemi2018fixing, huang2020augmented}), and \gls{RD} with additional sufficient statistics related to classification or generalization \cite{alemi2018therml, gao2020free}.  

\section{Background}\label{sec:background}
% We consider the representation learning scenario, where we would like to encode data $\x$ into a compressed latent code $\z$ which preserves information for unsupervised decoding or supervised classification \citep{alemi2018therml,gao2020free}, and discards information about sensitive attributes or nuisances \citep{moyer2018invariant,jaiswal2019discovery}. %,galstyan2020tradeoff}. %alemi2016deep,

\subsection{Exponential Family}\label{sec:exp_fam}
We slightly generalize the standard maximum entropy construction to include a base distribution $\pi_0(\z)$, where $\pi_0(\z) = 1$ or uniform corresponds to MaxEnt.  For a set of $M$ sufficient statistic functions $\phi(\x,\z) = \{\phi_j(\x,\z) \}_{j=1}^{M}$ and observed values $\mybar{\eta} =  \{\eta_j \}_{j=1}^{M}$ defining a feasible set of distributions $\mathcal{M}$,
\begin{align}
\min \limits_{q(\z|\x) \in \mathcal{M}} D_{KL}[q(\z|\x)||\pi_0(\z)] \quad \text{subj. to } \quad \mathbb{E}_{\, q(\z|\x)} [ \phi_j(\x, \z) ]= \eta_j \quad \forall j \label{eq:maxent}
\end{align}
The solution is given by distribution in the exponential family, where the $M$-dimensional vector of Lagrange multipliers $\beta = \{ \beta_j \}_{j=1}^M$ enforcing the constraints, corresponds to the natural parameter
\begin{align}  
\hfill \pi_{\beta} (\z|\x) &= \pi_0(\z) \exp \{ \, \sum \limits_{j=1}^{M} \beta_j \, \phi_j(\x, \z) - \psi(\beta) \, \} 
\quad \, \, \psi(\beta) = \log \int \exp \{ \, \sum \limits_{j=1}^{M} \beta_j \,\phi_j(\x, \z) \, \} \, d\z \label{eq:exp_fam} \, .
\end{align}
We will often write $\beta, \eta,$ and $\phi$ without vector notation, with equality conditions intended to hold in all dimensions.  For ease of notation, we write $\beta \cdot \eta = \sum \beta_j \, \phi_j(\x, \z) $ to imply the dot product.

Since the log partition function $\psi(\beta)$ is convex in $\beta$, its gradient will be unique and may be used as a dual parameterization of the distribution $\pi_{\beta}$ \citep{nielsen2009statistical,wainwrightjordan}, with components  
\begin{align}
\eta_j (\beta) = \frac{\partial \psi}{\partial \beta_j} = \mathbb{E}_{\pi_{\beta}} [ \phi_j(\x, \z)] \qquad \forall 1\leq j\leq M \label{eq:logpartition_deriv} \, .
\end{align}
so that each set of expected sufficient statistic constraints  $\eta_{\beta}$ corresponds to an entropy-maximizing solution $\pi_{\beta}$ \citep{wainwrightjordan}.


\subsection{Legendre Duality}\label{sec:legendre_background}
Since the log partition function $\psi(\beta)$ is a convex function of the natural parameters, we may also define its convex conjugate function $\psi^{*}$ using
%(\mybar{\eta})$, which takes as input any $\mybar{\eta}$ in the domain of the sufficient statistics.  This is also known as the Legendre transform, with %which incorporates all constraints.
\begin{align}
\psi^{*}(\omega) = \sup_{\beta} \beta \cdot \omega - \psi(\beta) \qquad \implies \omega_j &= \frac{\partial \psi}{\partial \beta} = \eta_j \, \, \forall \, \, j \label{eq:conjugate} %\mathbb{E}_{\pi_{\beta}} [ \phi_j(\x, \z) ]
% \psi^{*}(\mybar{\eta}) = \sup_{\beta} \beta \cdot \mybar{\eta} - \psi(\beta) \qquad \implies \mybar{\eta} = \frac{d\psi}{d\beta} = \mathbb{E}_{\pi_{\beta}} [ \phi(\x, \z) ] \label{eq:conjugate} 
\end{align}
This matches the condition in \eqref{eq:logpartition_deriv}, so that the supremum occurs when $\omega = \eta_{\beta} = d\psi / d\beta$ for appropriate choice of $\beta$.   Thus, we will proceed to write $\psi^{*}$ with the mean parameters $\eta_{\beta}$ or observed sufficient statistics $\bar{\eta}$ as its arguments.
\begin{align}
    \psi^{*}(\eta_{\beta}) = \beta \cdot \eta_{\beta} - \psi(\beta) \label{eq:legendre_sol}
\end{align}
With no base distribution, $\psi^{*}(\eta_{\beta})$ corresponds to the negative entropy of the maximum entropy solution $\pi_{\beta}$ with observable constraint $\eta_{\beta}$ \citep{wainwrightjordan}.  With a base distribution (e.g. \citep{brekelmans2020all} App. A), we have 
\begin{align}
\psi^{*}(\eta_{\beta}) = D_{KL}[\pi_{\beta}(\z|\x)||\pi_0(\z)] \label{eq:conjugate_kl}
\end{align}
Since $(\psi^{*})^{*} = \psi$, we can obtain a similar optimization to \eqref{eq:conjugate} in terms of $\psi(\beta) = \sup_{\eta} \beta \cdot \eta - \psi^{*}(\eta)$.  This leads to the canonical expression for Legendre duality, when the two optimizations are in equilibrium and the vectors $\eta_{\beta}$ and $\beta$ are in correspondence
\begin{align}
\psi^{*}(\eta_{\beta}) + \psi(\beta) - \beta \cdot \eta_{\beta} = 0 \, . \label{eq:legendre}
\end{align}
% With this expression, we may also rewrite \eqref{eq:exp_fam} using $\psi^{*}(\eta)$ as the normalizing constant.
% \begin{align}
% \pi_{\beta} (\z) &= \pi_0(\z) \exp \{ \, \sum \limits_{j=1}^{M} \beta_j \cdot \big( \phi_j(\x, \z) - \eta_j \big) + \psi^{*}(\eta_{\beta}) \, \} \label{eq:psi_exp_fam} %&= 
% \end{align}
%\pi_0(\z) \exp \{ \beta \cdot \phi(\z) - \psi(\beta) \} \nonumber \\[1.25ex]
%&= \pi_0(\z) \exp \{ \beta \cdot \phi(\z) - \beta \cdot \eta(\beta) + \psi^{*}(\eta(\beta)) \} \nonumber \\
% &= \pi_0(\z) \exp \{ \beta \, \big(\phi(\z) - \eta(\beta)\big) + \psi^{*}(\eta(\beta)) \} \label{eq:psi_exp_fam} %\\[1.25ex]
%&= \frac{\pi_0(\z) \exp \{ \beta \, \big(\phi(\z) - \eta(\beta)\big)}{\exp \{ - D_{KL}[\pi_{\beta} || \pi_0] \}}


==> sections/main/likelihood_ratio.tex <==

%%%
\section{Likelihood Ratio Exponential Family}\label{sec:lr_families}
We consider an exponential family of distributions with sufficient statistics $\phi(z) = \log \frac{\pi_1(z)}{\pi_0(z)}$ equal to the log likelihood ratio between two distributions of interest $\pi_0$ and $\pi_1$ \cite{brekelmans2020all}.  We can write this family $\pi_{\beta}$ using the natural parameter $\beta$ and base distribution $\pi_0$ as follows, 
\begin{align} %-d\textbf{}(\vx, \vz)
    \pi_{\beta}(\vz)  &= \pi_0(\vz) \exp \{ \beta  \cdot  \phi(\vz) \,   - \psi( \beta) \}  \label{eq:lkd_ratio_fam}  \\
    \phantom{\pi_{\beta}} \text{where } \, \, \phi(\vz)   :&= \log \frac{\pi_1(\vz)}{\pi_0(\vz)} \quad \quad \psi(\beta) := \log Z_{\beta} =  \log \int \pi_0(\vz)^{1-\beta} \pi_1(\vz)^{\beta} d\vz \label{eq:path_exp_family_general}
\end{align}
where, in writing $\psi(\beta)$ we note that \eqref{eq:lkd_ratio_fam} reduces to the geometric mixture $\pi_{\beta}(\vz) \propto \pi_0(\vz)^{1-\beta} \pi_1(\vz)^{\beta}$ for our choice of sufficient statistics.  Further, note the relationship of $\psi(\beta)$ to Rényi's $\alpha$ divergence \cite{renyi1961, van2014renyi} with order $\alpha = \beta$, so that $\psi(\beta) = (\beta - 1) D_{\beta}[\pi_1(\vz) || \pi_0(\vz)]$.

Intermediate distributions along the geometric mixture path can be given a variational representation as in \citet{grosse2013annealing}, with
\begin{align}
    \pi_{\beta_t}(\z) &= \argmin \limits_{r(\z)} (1-t) \, D_{KL}[ r(\z) || \pi_{\beta_0}(\z)] + \, t \, D_{KL}[  r(\z) || \pi_{\beta_1}(\z)] \, \label{eq:vrep1} \\
    & \text{where } \beta_t = (1-t) \cdot \beta_0 + t \cdot \beta_1  \quad \text{and } \pi_{\beta_t}(\z) \propto \pi_0(\vz)^{1-\beta_t} \pi_1(\vz)^{\beta_t} \nonumber %\\[2ex]
    % \pi_{\eta_t}(\z) &= \argmin \limits_{r(\z)} (1-t) \, D_{KL}[ \pi_{\beta_0}(\z) ||  r(\z)]  + \, t \, D_{KL}[ \pi_{\beta_1}(\z) || r(\z)] \label{eq:vrep2} \\
    % & \text{where } \eta_t = (1-t) \cdot \eta_0 + t \cdot \eta_1 \nonumber
\end{align}
In \cref{app:jensen_gaps}, we interpret this variational representation using a general result about Bregman divergences from \citet{Banerjee2005}. In particular, at the optimum above, the expected KL divergence reduces to a gap in Jensen's inequality for the function $\psi(\beta)$ with respect to the measure $\{ 1-t, t\}$ over $\{ \beta_0, \beta_1 \}$.  
\begin{align}
 (1-t) \, D_{KL}[ \pi_{\beta_t}(\z) || \pi_{\beta_0}(\z)] + \, t \, D_{KL}[ \pi_{\beta_t}(\z) || \pi_{\beta_1}(\z)] &= (1-t) \psi(\beta_0) + t \, \psi(\beta_1) - \psi( \beta_t )
\end{align}
As shown in \citet{nielsen2011renyi} or \cref{app:renyi}, Renyi's $\alpha$ divergence within an exponential family also corresponds to a gap in Jensen's inequality.   

In the next section, we will show that these variational representations are related to the asymptotic limit for the Neyman-Pearson lemma, which states that the likelihood ratio test is the optimal decision rule for a given acceptable error.















==> sections/main/rdc.tex <==
% !TEX root = main.tex
\section{A Free Energy Principle for Transfer Learning}\label{sec:fep}
\citet{gao2020free} build upon the general framework of \citet{alemi2018therml} for applications in transfer learning.   In particular, consider adding a classification loss with expectation constraint $C$ to the rate-distortion optimization for a \textit{single} representation $z$
\begin{align}
\min D_{KL}[q(\z|\x) || m(\z)] \quad \text{subj. to} \quad &\mathbb{E}_{q(\z | \x)} [ \log d(\x|\z) ] = -D := \eta_D \label{eq:fep} \\
& \mathbb{E}_{q(\z| \x)} [ \log c(y|\z)] = -C := \eta_C \nonumber \, .
\end{align}
We can view the classification loss as adding a sufficient statistic $\phi(y(\x), \z) = \log c(y|\z)$, with constraints written as negative to account for the additional factor in \eqref{eq:ba_sol}.   As in Eq. 9 of \citet{gao2020free}, the optimal encoder $q^{*}(\z|\x)$ becomes
\begin{align}
q^{*}(\z|\x) &=  m_0(\z) \exp \{ \lambda \cdot \log d(\x|\z) + \gamma \cdot \log c(y|\z) - \psi(\x; \lambda, \gamma) \} \\
&= \frac{1}{Z(\x; \lambda, \gamma)} \, \pi_0(\z) \,  d(\x|\z)^{\lambda} \, c(y|\z)^{\gamma}
\end{align}
where we use $\lambda$, $\gamma$ to enforce constraints on the distortion and classification losses, respectively. 
%match \cite{gao2020free}, and the Lagrange multiplier $\gamma$ enforces the constraint on the classification loss.  
We can then define the (expected) free energy across data samples as 
\begin{align}
 F( \lambda, \gamma) &= - \mathbb{E}_{q(\x)}[ \, \log Z(\x; \lambda, \gamma) \, ] = - \langle \, \psi(\x; \lambda, \gamma) \, \rangle_{q(\x)} \label{eq:fe} %\\
\end{align}
%We describe this in more detail in Sec. \textbf{tbd}. %\ref{sec:fep}

For a given $\lambda, \gamma$, \citet{gao2020free} denote $\nabla_{\theta} J_{\theta}(\theta, \beta) = - \mathbb{E}_{q(\x)} [ \nabla_{\theta}  \log Z(\x; \lambda, \gamma) \, ]$ for some (possibly non-equilibrium) value of network weights $\theta$, which encompass the encoder, classifier, and decoder.  Note that $\nabla_{\theta} J_{\theta}(\theta, \beta) = \nabla_{\theta} F(\lambda, \gamma) = 0$ if the current network achieves achieves optimality as a function of $q^{*}(\z|\x), \lambda, \gamma$.   \citet{gao2020free} refer to this as the `equilibrium surface', which we proceed to interpret in terms of Legendre duality.


\subsection{Legendre Duality Interpretation}
We can interpret the free energy in \eqref{eq:fep} using the Legendre duality of \eqref{eq:legendre}.  Recall that $\eta = \{ \eta_D, \eta_C \} = \{ -D, -C \}$, with the constraint values corresponding to the \textit{extensive} variables of the system \cite{alemi2018therml}.   As in \eqref{eq:rate_psi}, the rate $R$ corresponds to $\psi^{*}(\eta_D, \eta_C)$, which we write more explicitly as the optimum of the dual optimization $\psi^{*}(\eta) = \sup_{\beta} \beta \cdot \eta - \psi(\beta)$ for $\beta = \{\lambda, \gamma \} $
\begin{align}
R(D,C) = \psi^{*}(\eta_D, \eta_C) = \sup \limits_{\lambda^{\prime}, \gamma^{\prime} } - \lambda^{\prime} \, D - \gamma^{\prime} \, C - \psi(\lambda^{\prime}, \gamma^{\prime})
\label{eq:leg} \end{align}
The rate $R = \psi^{*}(\eta_D, \eta_C)$ is thus associated with the expectation constraints $\{ -D, -C \}$. At equilibrium or optimality in \eqref{eq:leg} ,  $\lambda = \lambda^{*}$ and $\gamma = \gamma^{*}$ correspond to the \textit{intensive variables}, which enforce the constraints and induce a log partition function of $\psi(\lambda, \gamma)$, which normalizes  \eqref{eq:ba_sol}.  

Alternatively, the free energy is the solution to an optimization as in Eq. 9 of \citet{gao2020free}
\begin{align}
  -F(\lambda, \gamma)=  \psi(\lambda, \gamma) = \sup_{D,C} - \lambda \, D - \gamma \, C - \psi^{*}(\eta_D, \eta_C) \label{eq:fe}
\end{align}
For fixed $\lambda, \gamma$, we can optimize \eqref{eq:fe} via the parameters $\theta$ until reaching the appropriate $D, C$.  

Lemma 3 of \citet{gao2020free} is obtained from the convexity of  $\psi(\lambda, \gamma)$ and $\psi^{*}(\eta_D, \eta_C)$.


On the equilibrium surface, we obtain the same form as \eqref{eq:legendre}, with $-F = \psi(\lambda, \gamma)$, $R = \psi^{*}(D,C)$, and $D, C$ corresponding to the sufficient statistics $\eta$
\begin{align}
 \psi^{*}(D, C) + \psi(\lambda, \gamma) - \lambda \, \eta_D - \gamma \, \eta_C = 0 \, . \label{eq:legendre_dc}
\end{align}
  See footnote for a minor confusion here. \footnote{\citet{alemi2018therml} view \eqref{eq:legendre_dc} as defining the feasible constraint set linking the values of each functional $R, D, C$.  Rearranging and taking the differential of $\psi^{*}(\eta_D, \eta_C)= R$, \cite{alemi2018therml,gao2020free} state a `conservation of information' analogue of the first law of thermodynamics
\begin{align}
d \psi^{*} = dR = -\frac{\partial R}{\partial D} dD - \frac{\partial R}{\partial C} dC = - \lambda \, dD - \gamma \, dC = \lambda \, d\eta_{D} + \gamma \, d\eta_C
\end{align}
Similarly to \eqref{eq:conjugate}, notice that the each partial of the conjugate, e.g. $\frac{\partial }{\partial \eta_D}\psi^{*}(\eta) = - \partial R / \partial D  = \lambda$ equals a natural parameter, e.g. $\lambda$, with $\eta_D = -D$.   RB isn't sure why this wouldn't include partials like $\frac{\partial }{\partial D} \psi(\beta), \frac{\partial }{\partial C} \psi(\beta)$.  Do \citet{gao2020free}\cite{alemi2018therml} implicitly consider `conservation' for a fixed free energy $\psi(\lambda, \gamma)$ so that $d\psi = 0$?} 


We can use Bregman divergences associated with the free energy $-F = \psi$ and rate $R = \psi^{*}$ to derive simple expressions for the KL divergence between distributions on the equilibrium surface.  See \citet{brekelmans2020tvo} Sec. 4.1 or App. A for details.  Again letting $\beta = \{\lambda, \gamma \}$ and $\beta^{\prime} = \{\lambda^{\prime}, \gamma^{\prime} \}$
\begin{align}
    D_{KL}[\pi_{\beta} || \pi_{\beta^{\prime}}] = D_{\psi}[\beta^{\prime} : \beta] &=  \psi(\lambda^{\prime},  \gamma^{\prime} ) - \psi(\lambda, \gamma)  - ( \lambda^{\prime}  - \lambda )\cdot (-D_{\beta})  \nonumber \\
    &\phantom{=  \psi(\lambda^{\prime} , \gamma^{\prime} ) - \psi(\lambda, \gamma) } \, \, - ( \gamma^{\prime}  -  \gamma)\cdot (-C_{\beta}) \\[2ex]
    = D_{\psi^{*}}[\eta_{\beta}: \eta_{\beta^{\prime}}] &=  \psi^{*}(D_{\beta^{\prime}}, C_{\beta^{\prime}}) - \psi^{*}(D_{\beta}, C_{\beta})  - (-D_{\beta} + D_{\beta^{\prime}}) \cdot \lambda{\prime}  \nonumber \\
    & \phantom{=  \psi^{*}(D_{\beta^{\prime}}, C_{\beta^{\prime}}) - \psi^{*}(D_{\beta}, C_{\beta}) } \, - (-C_{\beta} + C_{\beta^{\prime}}) \cdot \gamma^{\prime}
\end{align}
where the Bregman divergence is defined as $D_f[a:b] = f(a) - f(b) - \langle a-b,  \nabla f(b) \rangle $ where $\langle x, y \rangle$ indicates the dot product over vectors.  Also note that $D = -\eta_{D}$.



\subsection{Partial Legendre Transforms}

\citet{alemi2018therml} consider `partial' Legendre transforms to derive various Maxwell relations.   RB doesn't have extensive background in physics, but this may spark additional intuitions.

It appears that a partial transform corresponds to a functional over a \textit{combination} of intensive and extensive variables.  For example, the iso-classification process might correspond to $G(\lambda, C)$, i.e. fixing the classification loss at a given value $C$ and optimizing with Lagrange multiplier $\lambda$ until we reach the equilibrium surface.  Note that this is not the same as either of the above, since we do not know the resulting equilibrium distortion $D_{\lambda}$, and may need to update the classification Lagrange multiplier $\gamma$.   

This might also be a useful construction in the DSF setting if we want to, for example, optimize the supervised representation $z_s$ for a Lagrange multiplier $\gamma$ and fixed distortion constraint $D$.


 
%  \begin{figure}[t]
% \includegraphics[trim=10 0 10 0, clip, width=\textwidth]{figs/fep_cifar.png}
% \caption{Iso-Classification Process on CIFAR10.  Models are first trained with given Lagrange multipliers for 120 epochs.  The Lagrange multipliers $\lambda, \gamma$ are changed, with their dynamics linked via Eq. 31 of \citet{gao2020free}, and the parameters $\theta$ are updated to try to reach the equilibrium surface ($\nabla_{\theta} F =0$) after each change in $(\lambda, \gamma)$.  Note that this results in both $\lambda$ and $\gamma$ increasing, and both $R$ and $D$ increasing with constant $C$.  This indicates that there is competition between what information to include in the representation $\z$, so that increasing $\lambda$ to lower distortion comes at the cost of higher supervised loss $C$.  The iso-classification process thus alternates between prioritizing reconstruction $D$ and label prediction $C$.} \label{fig:fep_cifar}
% \end{figure}

% \subsection{Reaching the Equilibrium Surface}
% Note that the dual optimizations of $\psi(\lambda, \gamma)$ or $\psi^{*}(D, C)$ are in terms of the Lagrange multipliers or constraints, respectively.  It is usually difficult to specify $D$ and $C$ without first training to convergence with a given $\lambda$ or $\gamma$.   

% \citet{gao2020free} identify reaching the equilibrium surface for a given $\beta = \{ \lambda, \gamma\}$ as having $\nabla_{\theta} J(\beta) = \nabla_{\theta} F(\beta) = 0$, and then propose \textit{quasi-static} dynamics which which evolve the parameters $\theta$ to maintain this condition
% \begin{align}
% \text{Equilibrium Surface} &\quad \nabla_{\theta} J_{\theta}(\theta, \beta) = \mathbb{E}_{q(\x)} \nabla_{\theta} \log Z(x; \lambda, \gamma) = 0  \label{eq:eq_surface} \\ 
% \text{Quasi-Static:}  &\quad \frac{d}{dt} \nabla_{\theta} J_{\theta}(\theta, \beta) = 0 \label{eq:quasi} \, .
% \end{align}
% Note that dynamics on the Lagrange multipliers $\dot{\lambda} = \frac{d \lambda}{dt}, \dot{\gamma} =  \frac{d \gamma}{dt}$ must also be specified (Lemma 5 \cite{gao2020free}).

% \subsection{Partial Legendre Transform?} 
% Upon reaching the equilibrium surface, the natural parameters $\beta = \{ \lambda, \gamma\}$ and $\eta = \{D, C\}$ are in dual correspondence \eqref{eq:legendre_dc}.  We may thus shift to specifying our optimization in terms of the constraint values, with some $f(R,D,C)=0$ defining the equilibrium surface allowing us to write each functional in terms of the others.   For example, we can write the Legendre transform $R(D,C) = \psi^{*}( D,C) = -\lambda \cdot D - \gamma \cdot C - \psi(\beta)$ as in \eqref{eq:legendre_dc} or \cite{alemi2018therml,gao2020free}.

% \citet{alemi2018therml} also consider `partial' Legendre transforms, which give rise to various Maxwell Relations. \footnote{See their ICLR submission \href{https://openreview.net/forum?id=HJeQToAqKQ}{App. F (at link here)} exploring more partial transforms than arXiv version.}  Rob doesn't fully understand this, but it appears that this defines \textit{mixed} functionals involving both constraints and Lagrange multipliers.  

% %For example, perhaps iso-classification might be understood in these terms, with a new functional $\Psi$ analogous to the \textit{free rate} in \cite{alemi2018therml}.  Keeping constant $C^{(t)}$ and changing $\beta^{(t)}_d$ from an equilibrium $\beta^{(t-1)}_D$, we might define 
% %\begin{align}
% %\Psi(C, \beta^{(t)}_d) = \sup \limits_{\theta} \, \beta^{(t)}_d \cdot \mathbb{E}_{q_{\theta}}[\log p(\x|\z)]  - R \quad \text{subject to} \quad  \mathbb{E}_{q_{\theta}}[\log c(y|\z) ] = C
% %\end{align}

% % let us denote $\eta_{D,\theta} = \mathbb{E}_{q_{\theta}}[\log p(\x|\z)]$ for some non-equilibrium parameters, so that we seek to find the equilibrium $D_{\theta} = \eta_{\lambda}$ for our new value of $\lambda$ 
% % \begin{align}
% %     \Psi(C, \lambda) = \sup \limits_{q_{\theta}(z|x)} -\lambda   - \psi^{*} = \sup -\lambda \cdot D_{\theta}  - R \, .
% % \end{align}


% %of a constraint $C$, which is referred to as the \textit{iso-classification} process \cite{gao2020free}.
% \subsection{Iso-Classification Process} 


% %After doing so, \citet{gao2020free}






% %  %with respect to parameters $\theta$.    
% % For a given $\lambda, \gamma$, \citet{gao2020free} denote $\nabla_{\theta} J_{\theta}(\theta, \beta) = - \mathbb{E}_{q(\x)} [ \nabla_{\theta}  \log Z(\x; \lambda, \gamma) \, ]$ for some (possibly non-equilibrium) value of network weights $\theta$, which encompass the encoder, classifier, and decoder.  Note that $\nabla_{\theta} J_{\theta}(\theta, \beta) = \nabla_{\theta} F(\lambda, \gamma)$ if the current network achieves achieves optimality as a function of $q^{*}(\z|\x), \lambda, \gamma$.   \citet{gao2020free} refer to this as the `equilibrium surface'.

% \citet{gao2020free} propose to evolve the Lagrange multipliers according to an `iso-classification' condition  
% \begin{align}
% \text{Iso-Classification:} &\quad \frac{dC}{dt} = 0 \label{eq:iso_clf} .
% \end{align}
% This implies dynamics on the Lagrange multipliers to keep the free energy constant, \footnote{\textcolor{red}{Rob had a slight confusion with the derivation...} In derivations starting from $\frac{dC}{dt} = 0$ in App. D, it seems like the terms  $\dot{\theta} \nabla_{\theta} C$ are ignored, i.e. the dynamics in \eqref{eq:lagr_updates} fulfill the condition $\frac{dC}{dt} = 0$ with $\dot{\theta} \nabla_{\theta} C = 0$.  I would have expected }  with $\alpha >0 $ taken to be a scaling parameter
% \begin{align}
% \frac{d \lambda}{d t} = -\alpha \frac{\partial C}{\partial \gamma} \qquad  \frac{d \gamma}{d t} = \alpha \frac{\partial C}{\partial \lambda} \label{eq:lagr_updates}.
% \end{align}
% \citet{gao2020free} convincingly apply the iso-classification process for preserving performance while transferring to new datasets, fine-tuning the model along a mixture path $(1-t) \, q(\x) + t \, q_t(\x)$ between training data $q(\x)$ and a transfer or target dataset $q_t(\x)$.


% For the case of a static dataset in Figure \ref{fig:fep_cifar}, evolving the dynamics in \eqref{eq:eq_surface}-\eqref{eq:iso_clf} result in the the model exploring the entire R-D curve for a constant C.  The Lagrange multipliers both increase throughout much of the iso-classification process, indicating a competition between reconstruction and classification information in the latent representation $\z$.
%  In particular, $\frac{d \gamma}{d t} > 0$ indicates that $\frac{\partial C}{\partial \lambda}$ is positive in practice, so that emphasizing lower distortion ($ \lambda \uparrow $) results in worse classification performance ( $\lambda \downarrow$).  See Figure \ref{fig:fep_cifar} caption for more details.  

% It is not clear it is desirable to raise the rate and lower the distortion for a constant (and possibly low) classification loss.   Instead, we might like to balance these competing objectives, so that we can increase classification performance, lower the rate, and lower distortion.   To separate these potentially competing objectives, we consider equilibrium dynamics for the \gls{DSF} framework in Sec. \ref{sec:fep_dsf}.

% %However, for the case of a static dataset, the conditions in \eqref{eq:eq_surface}-\eqref{eq:iso_clf} give undesirable results in Figure \ref{fig:fep_cifar}.  In particular, both $\lambda$ and $\gamma$ appear to increase over the course of the iso-classification process, which raises the rate $R$ and lowers the distortion $D$ for a constant $C$.  
% % In particular, the Lagrange multipliers both increase throughout much of the iso-classification process.
% % This indicates a competition between reconstruction and classification information in latent $\z$, which should be naturally addressed by learning separate representations in \gls{DSF} in Sec. \ref{sec:fep_dsf}.  In particular, $\frac{d \gamma}{d t} > 0$ indicates that $\frac{\partial C}{\partial \lambda}$ is positive in practice, so that emphasizing lower distortion ($ \lambda \uparrow $) results in worse classification performance ( $\lambda \downarrow$).  See Figure \ref{fig:fep_cifar} caption for more details.  


% % \subsection{Legendre Duality}
% % We can interpret the free energy in \eqref{eq:fep} using the Legendre duality of \eqref{eq:legendre}.  Recall that $\eta = \{ \eta_D, \eta_C \} = \{ -D, -C \}$, with the constraint values corresponding to the \textit{extensive} variables of the system \cite{alemi2018therml}.   As in \eqref{eq:rate_psi}, the rate $R$ corresponds to $\psi^{*}(\eta_D, \eta_C)$, which we write more explicitly as the optimum of the dual optimization $\psi^{*}(\eta) = \sup_{\beta} \beta \cdot \eta - \psi(\beta)$
% % \begin{align}
% % R(D,C) = \psi^{*}(\eta_D, \eta_C) = \sup \limits_{\lambda, \gamma} -\lambda \, D - \gamma \, C - \psi(\lambda, \gamma) 
% % \end{align}
% % The rate $R = \psi^{*}(\eta_D, \eta_C)$ is thus associated with the expectation constraints $\{ -D, -C \}$. At equilibrium,  $\lambda = \beta_{d^*}$ and $\gamma = \beta_{c^*}$ correspond to the \textit{intensive variables}, which enforce the constraints and induce a log partition function of $\psi(\lambda, \gamma)$, which normalizes  \eqref{eq:ba_sol}.  

% % Alternatively, the free energy can be viewed as an optimization, as in Eq. 9 of \citet{gao2020free}
% % \begin{align}
% %   F(\lambda, \gamma)=  \psi(\lambda, \gamma) = \sup_{D,C} - \lambda \, D - \gamma \, C - \psi^{*}(\eta_D, \eta_C) \label{eq:fe}
% % \end{align}
% % For fixed $\lambda, \gamma$, we can optimize \eqref{eq:fe} via the parameters $\theta$ until reaching the appropriate $D, C$.   


% % On the equilibrium surface, we obtain the same form as \eqref{eq:legendre}, with $F = \psi(\lambda, \gamma)$, $R = \psi^{*}(D,C)$, and $D, C$ corresponding to the sufficient statistics $\eta$
% % \begin{align}
% %  \psi^{*}(\eta_D, \eta_C) + \psi(\lambda, \gamma) - \lambda \, \eta_D - \gamma \, \eta_C = 0 \, . \label{eq:legendre_dc}
% % \end{align}
% %   See footnote for an minor confusion here. \footnote{\citet{alemi2018therml} view \eqref{eq:legendre_dc} as defining the feasible constraint set linking the values of each functional $R, D, C$.  Rearranging and taking the differential of $\psi^{*}(\eta_D, \eta_C)= R$, \cite{alemi2018therml,gao2020free} state a `conservation of information' analogue of the first law of thermodynamics
% % \begin{align}
% % d \psi^{*} = dR = -\frac{\partial R}{\partial D} dD - \frac{\partial R}{\partial C} dC = \lambda \, dD + \gamma \, dC
% % \end{align}
% % In similar fashion to \eqref{eq:conjugate}, we can notice that the partial of the conjugate $\frac{\partial \psi^{*}(\eta)}{\partial \eta_D} = -\frac{\partial R}{\partial D} = \lambda$, where $\psi^{*}$ is a function of the moment parameters, equals the natural parameter.  \textcolor{red}{There appears to be a problem, though.} I'm not sure why this wouldn't include partials like $\frac{\partial }{\partial D} \psi(\beta), \frac{\partial }{\partial C} \psi(\beta)$.  Do \citet{gao2020free} and \citet{alemi2018therml} consider this for a fixed free energy $\psi(\lambda, \gamma)$ so that $d\psi = 0$?} 





% %We can consider the iso-classification process using a partial Lagrangian, where we fix the classification constraint $C$ and relax the distortion constraint $\lambda \, D$.  
% %Similar to the first law of learning, \citet{alemi2018therml}'s `Maxwell Relations' allow us to define 
% %we fix the constraint $C$ rather than the Lagrange multiplier $\gamma$.

% %In the context of \gls{DSF} in Sec. \ref{sec:fep_dsf}, it may be useful to consider `partial' Legendre transforms, where we update only a subset of the $\beta_j, \eta_j$ pairs along the equilibrium surface (see \citet{alemi2018therml} Sec. 3.2, or  \href{https://openreview.net/forum?id=HJeQToAqKQ}{Appendix F (at link here)}).


==> sections/main/variational_rep.tex <==
\section{Variational Representation}\label{sec:vrep}
For the case of the geometric and moment mixtures found in \gls{TVO}, \citet{grosse2013annealing} mention the following variational representation of intermediate distributions.
\begin{align}
    \pi_{\beta_t}(\z) &= \argmin \limits_{r(\z)} (1-t) \, D_{KL}[ r(\z) || \pi_{\beta_0}(\z)] + \, t \, D_{KL}[  r(\z) || \pi_{\beta_1}(\z)] \label{eq:vrep1} \\
    & \text{where } \beta_t = (1-t) \cdot \beta_0 + t \cdot \beta_1 \nonumber \\[2ex]
    \pi_{\eta_t}(\z) &= \argmin \limits_{r(\z)} (1-t) \, D_{KL}[ \pi_{\beta_0}(\z) ||  r(\z)]  + \, t \, D_{KL}[ \pi_{\beta_1}(\z) || r(\z)] \label{eq:vrep2} \\
    & \text{where } \eta_t = (1-t) \cdot \eta_0 + t \cdot \eta_1 \nonumber
\end{align}
Considering the KL divergence as a Bregman divergence $D_{\psi}[\beta_0 : \beta_1] = D_{KL}[\pi_{\beta_1} || \pi_{\beta_0} ]$ and $D_{\psi^{*}}[ \eta_0 : \eta_1] = D_{KL}[\pi_{\eta_0} || \pi_{\eta_1}] = D_{KL}[\pi_{\beta_0} || \pi_{\beta_1}]$% \footnote{Note that any exponential family distribution can be indexed by either the natural or moment parameters, e.g. $\beta_0$ or $\eta_0$.}
, we can see that this is a special case of a result from \citet{Banerjee2005}.  In particular, with respect to a particular measure (e.g. $p_0 = 1-t, p_1 = t $), the mean of the arguments (either $\{\beta_0, \beta_1\}$ or $\{\eta_0, \eta_1\}$) minimizes the expected Bregman divergence to a single point in the second argument.  
\begin{align}
     \mathcal{J}_{F, p(x_i)} :&= \min \limits_{x^{*}} \mathbb{E}_{p(x_i)} \big[ D_{F}[ x_i || x^{*} ] \big]  \quad \text{with} \quad \mu := \argmin \limits_{x^{*}} \mathcal{J}_{f, p(x_i)} = \mathbb{E}_{p(x_i)}[\, x^{*} \,] 
\end{align}
At this minimum, the expected Bregman divergence $D_F$ corresponds to the gap in Jensen's inequality for the function $F$ with respect to the measure $p(x_i)$
\begin{align}
      \mathcal{J}_{F, p(x_i)} {}  &= \mathbb{E}_{p(x_i)}[ \, F(x_i) \, ] - F(\mathbb{E}_{p(x_i)}[x_i]) = \mathbb{E}_{p(x_i)}[ \, F(x_i) \, ] - F(\mu) \, .
\end{align}
We now provide two examples of this expected Bregman divergence.


For the case of the \gls{TVO} geometric mixture family and the variational representations in \eqref{eq:vrep1}-\eqref{eq:vrep2}, we can consider a path between $\beta_0$ and $\beta_1$ according to a parameter $t$, with  $\mu_{\beta, t} = (1-t) \beta_0 + t\, \beta_1$.  For $\beta_0 = 0$ and $\beta_1 = 1$, we obtain  $\mu_{\beta, t} = \beta$, and
\begin{align}
 \mathcal{J}_{\psi, \{ 1-t, t \}} &= (1-t) \, D_{\psi}[\beta_0 : \mu_{\beta,t}] + t \, D_{\psi}[\beta_1 : \mu_{\beta,t}] \\
 &= (1-t) \, D_{KL}[ \pi_{\beta} : \beta_0 ] + t \, D_{KL}[\pi_{\beta} : \beta_1] \label{eq:jg_kl} 
\end{align}
to match the variational representation in \eqref{eq:vrep1}.  Since $D_{KL}$ is a Bregman divergence $D_{\psi}$, we can simplify or use \citet{Banerjee2005} to write this as a gap in Jensen's inequality for the convex function $\psi(\beta)$ and expectations wrt $(1-t), t$
\begin{align}
 \mathcal{J}_{\psi, \{ 1-t, t \}} &= (1-t) \, \psi(\beta_0) + t \, \psi(\beta_1) - \psi \big( \mu_{\beta,t} \big) \label{eq:jg_psi}
\end{align}
Finally, the Renyi $\alpha$-divergence within an exponential family corresponds to a gap in Jensen's inequality as shown in \citet{nielsen2011renyi} or on the next page, so that
\begin{align}
\mathcal{J}_{\psi, \{ 1-t, t \}} &= (1-t) \, D_{t}[\pi_{\beta_1} : \pi_{\beta_0} ] \label{eq:jg_renyi}
\end{align}

The variational representation of the moment-averaging curve \eqref{eq:vrep2} can also be viewed as a gap in Jensen's inequality using the dual divergence $D_{\psi^*}$, which simply reverses the order of arguments
\begin{align}
     \mathcal{J}_{\psi^{*}, \{ 1-t, t \}} &= (1-t) \, D_{\psi^{*}}[\eta_0 : \mu_{\eta,t}] + t \, D_{\psi^{*}}[\eta_1 : \mu_{\eta,t}] \\
 &= (1-t) \, D_{KL}[ \pi_{\eta_0} : \pi_{\mu_{\eta,t}} : ] + t \, D_{KL}[\pi_{\eta_1} : \pi_{\mu_{\eta,t}}] \\
 &= (1-t) \, \psi^{*}(\eta_0) + t \, \psi^{*}(\eta_1) - \psi^{*} \big( \mu_{\eta,t} \big)
\end{align}


==> sections/new_main/0_intro.tex <==
% \section{Introduction}
% The exponential family is well known in machine learning and statistical physics as the maximum entropy distribution subject to a set of observed constraints \cite{jaynes1957information}, while the geometric mixture path is common in \textsc{mcmc} methods such as \gls{AIS} \cite{neal2001annealed, jarzynski1997equilibrium}.   Linking these two ideas, \citet{brekelmans2020all} interpret the geometric mixture path as an exponential family of distributions to analyse the recent \gls{TVO} \cite{masrani2019thermodynamic}.  

% In this work, we extend \textit{likelihood ratio exponential families} to include solutions to \gls{RD} optimization \cite{alemi2018fixing, cover2012elements}, the \gls{IB} method \cite{tishby1999information}, and recent `\textsc{rdc}' approaches which combine \gls{RD} and \gls{IB} \cite{gao2020free, alemi2018therml},  providing a common mathematical framework for understanding these methods via the conjugate duality of exponential families and hypothesis testing.  We collect existing results \cite{Banerjee2005, grosse2013annealing, nielsen2013information, borade2006projection} to provide a variational representation of intermediate \gls{RD} or \gls{TVO} distributions as a minimizing an expectation of \textsc{kl} divergences.  This solution also corresponds to an optimal decision test using the Neyman Pearson lemma.   In \gls{TI} \cite{ogata1989monte, gelman1998simulating} bounds such as those in the \gls{TVO}, we identify the critical point of these optimizations as the
% intermediate distribution whose expected sufficient statistics match the log partition function.
 
% % We leverage these perspective to identify , may be constructed for any likelihood ratio family, and identify the point where the moment constraint matches the log partition function.
  
% %  an expected \textsc{kl} divergence related to hypothesis testing and the Neyman Pearson lemma \cite{cover2012elements, csiszar2004information}.  Finally, we highlight that \gls{TI} \cite{ogata1989monte, gelman1998simulating} bounds, such as those found in the \gls{TVO}, may be constructed for any likelihood ratio family, and identify the point where the moment constraint matches the log partition function.
% % %expected sufficient statistics, or distortion, 
% %gls{TVO} or \gls{RD}




% % In this paper, we analyze \textit{likelihood ratio} exponential families \cite{brekelmans2020all}, which can be constructed between arbitrary distributions that are not themselves in exponential family form, from the point of view of Legendre duality and hypothesis testing. This yields a common mathematical framework for understanding methods such as the \gls{TVO} \cite{masrani2019thermodynamic, brekelmans2020all}, \gls{RD} optimization \cite{alemi2018fixing}, and recent `\textsc{rdc}' approaches \cite{gao2020free, alemi2018therml} that include a classification loss as in the \gls{IB} \cite{tishby1999information}. %additional




% % The exponential family is well known in machine learning and statistical physics as the maximum entropy distribution subject to a set of observed constraints \cite{jaynes1957information}, while the geometric mixture path is common in \textsc{mcmc} methods such as \gls{AIS} \cite{neal2001annealed, jarzynski1997equilibrium}.   Linking these two ideas, \citet{brekelmans2020all} interpret the geometric mixture path as an exponential family of distributions to analyse the recent \gls{TVO} \cite{masrani2019thermodynamic}.  

% % %which combine
% % In this work, we extend \textit{likelihood ratio exponential families} to include solutions to \gls{RD} optimization \cite{alemi2018fixing, cover2012elements}, the \gls{IB} method \cite{tishby1999information}, and recent rate-distortion-classification (\textsc{rdc}) approaches combining \gls{RD} and \gls{IB} \cite{gao2020free, alemi2018therml}.  We provide a common mathematical framework for understanding these methods using the conjugate duality of exponential families.  Further, we collect existing results \cite{grosse2013annealing, Banerjee2005, nielsen2013information} to express intermediate distributions via a variational representation  related to hypothesis testing and the Neyman Pearson lemma \cite{borade2006projection, csiszar2004information}, and leverage this perspective to identify the point at which the \gls{TVO} integrand, or expected likelihood ratio, matches the log partition function.  %bounds may be constructed for any likelihood ratio family, and identify the point where the 
% % %Finally, we highlight that \gls{TI} \cite{ogata1989monte, gelman1998simulating} bounds, such as those found in the \gls{TVO}, may be constructed for any likelihood ratio family, and identify the point where the expected likelihood ratio, or moment constraint, matches the log partition function.

==> sections/new_main/1_zlegendre.tex <==
\section{Legendre Duality}\label{sec:duality}
%\subsection{Legendre Duality}\label{sec:legendre_background}
Since the log partition function $\psi(\beta)$ of an exponential family is convex in the natural parameters $\beta$, its gradient will be unique and may be used as a dual parameterization for $\pi_{\beta}$ \citep{nielsen2009statistical,wainwrightjordan}.  This correspondence between the \textit{natural} parameters $\beta = \{ \beta_j \}$ and \textit{moment} parameters, denoted $\eta = \{ \eta_j \}$, also defines the convex conjugate function $\psi^{*}(\eta)$, with
\begin{align}
\psi^{*}(\eta) = \sup_{\beta} \beta \cdot \eta - \psi(\beta) \qquad \implies \eta_j &= \frac{\partial \psi}{\partial \beta}= \mathbb{E}_{\pi_{\beta}} [ \phi_j(\x, \z)] \, \, \forall \, \, j \label{eq:conjugate} 
% \eta_j (\beta) = \frac{\partial \psi}{\partial \beta_j} = \mathbb{E}_{\pi_{\beta}} [ \phi_j(\x, \z)] \qquad \forall 1\leq j\leq M \label{eq:logpartition_deriv} \, .
\end{align}
With the Lebesgue or counting measure, $\psi^{*}(\eta)$ corresponds to the negative entropy of the maximum entropy solution $\pi_{\beta}$ with observable constraint $\eta$ \citep{amari2016information, wainwrightjordan}.  With a general base distribution (e.g. \citep{brekelmans2020all} App. A), we have 
\begin{align}
\psi^{*}(\eta_{\beta}) = D_{KL}[\pi_{\beta}(\z|\x)||\pi_0(\z)] \label{eq:conjugate_kl}
\end{align}
Since the convex conjugate is an involution, $(\psi^{*})^{*} = \psi$, we can obtain a similar optimization to \eqref{eq:conjugate} in terms of $\psi(\beta) = \sup_{\eta} \beta \cdot \eta - \psi^{*}(\eta)$.  This leads to the canonical expression for Legendre duality, when the two optimizations are in equilibrium and the vectors $\eta_{\beta}$ and $\beta$ are in correspondence \cite{amari2016information}
\begin{align}
\psi^{*}(\eta_{\beta}) + \psi(\beta) - \beta \cdot \eta_{\beta} = 0 \, . \label{eq:legendre}
\end{align}
We can also construct a Bregman divergence, which corresponds to the gap in a first order Taylor approximation, using any convex function.  For example, using $\psi(\beta)$ or $\psi^{*}(\eta)$, we have
\begin{align*}
\begin{adjustbox}{max width=\textwidth}
\begin{aligned}
  D_{\psi}[\beta : \beta^{\prime}] = \psi(\beta) - \psi(\beta^{\prime}) - \langle \beta - \beta^{\prime}, \nabla \psi(\beta^{\prime}) \rangle
\end{aligned}\hspace*{.5cm}
\begin{aligned}
  D_{\psi^{*}}[\eta : \eta^{\prime}] = \psi^{*}(\eta) - \psi^{*}(\eta^{\prime}) - \langle \eta - \eta^{\prime}, \nabla \psi^{*}(\eta^{\prime}) \rangle
\end{aligned}
\end{adjustbox}
\end{align*}
Using the duality relationship \eqref{eq:legendre} and definition of the exponential family, we can see that \cite{ brekelmans2020all}
\begin{align}
     D_{\psi}[\beta : \beta^{\prime}] = D_{\psi^{*}}[ \eta_{\beta^{\prime}}: \eta_{\beta} ] = D_{KL}[ \pi_{\beta^{\prime}} || \pi_{\beta} ] \label{eq:divergences}
\end{align}

%\section{Rate-Distortion Examples}\label{sec:rd_duality}
\paragraph{Duality in Rate-Distortion} 


Similar expressions are discussed in \citet{rose1990deterministic}.

\paragraph{\gls{RDC} Case:}

==> sections/new_main/3_rdc.tex <==
\section{Multiple Sufficient Statistics}\label{sec:rdc}
Several recent works \cite{gao2020free,alemi2018therml} consider both distortion and classification loss, which we denote as `\textsc{rdc}' %, for applications in transfer learning %an optimization which we reference as \gls{RDC}, 
\begin{align}
\min \limits_{q(\vz|\vx)} D_{KL}[q(\z|\x) || m(\z)] \quad \text{subj. to} \quad &\mathbb{E}_{q(\z | \x)} [ d(\x,\z) ] \leq D \, \, , \, \, \mathbb{E}_{q(\z| \x)} [ c(y, \z)] \leq C  \label{eq:fep1} 
\end{align}
In this case, we may consider \textit{two} sufficient statistics in our likelihood ratio exponential family.  Similarly to \citet{Slonim2006}, we use an unnormalized target which factorizes as $\tilde{\pi}_1(\vx,y,\vz) = p_{\theta}(\vx|\vz) p_{\theta}(y, \vz)m(\vz)$, and consider the likelihood ratio sufficient statistics
\begin{align}
\begin{adjustbox}{max width=\textwidth}
\begin{aligned}
    \phi_d(\vx, \vz) = \log \frac{\pi_1(\vz|\vx)}{\pi_0(\vz)} = \log \frac{ p_{\theta}(\vx|\vz)}{\px} \propto -d(\vx, \vz) \label{eq:rdc_phi}
\end{aligned}\hspace*{.5cm}
\begin{aligned}
      \phi_c(y, \vz) = \log \frac{\pi_1(\vz|y)}{\pi_0(\vz)} = \log \frac{ p_{\theta}(y, \vz)}{p(y)} \propto \log p_{\theta}(y|\vz) = -c(y, \vz)
\end{aligned}
\end{adjustbox}
\end{align}
where we again absorb $\px$ and $p(y)$ into the normalization, using $\phi_d(\vx,\vz) = -d(\vx, \vz)$ as in \eqref{eq:phi_d}.
Introducing Lagrange multipliers $\beta = \{\beta_c, \beta_d\}$ as in \eqref{eq:q_star_rd}, we obtain the solution of \eqref{eq:fep1} as a geometric mixture \cite{gao2020free, alemi2018therml}, belonging to the likelihood ratio exponential family with $\phi = \{\phi_d, \phi_c\}$ \eqref{eq:rdc_phi}
\begin{align}
\begin{adjustbox}{max width=\textwidth}
    \pi_{\beta}(\vz|\vx,y) =  m(\z) \exp \{ \beta_D \cdot \phi_d(\vx|\vz) + \beta_C \cdot \phi_c(y|\vz) - \psi(\x, y; \beta) = \frac{1}{Z_{\beta}(\x,y)} \, m(\z) \, p_{\theta}(\vx|\vz)^{\beta_D} \,p_{\theta}(y|\vz)^{\beta_C}  \nonumber
    %m_0(\z) \exp \{ \lambda \cdot \log d(\x|\z) + \gamma \cdot \log c(y|\z) - \psi(\x; \lambda, \gamma)
\end{adjustbox}
\end{align}
where $\beta_D, \beta_C$ reflect the optimal set of Lagrange multipliers $\beta$ enforcing $D = -\eta_{d}(\beta)$, $C = -\eta_{c}(\beta)$.
%match \cite{gao2020free}, and the Lagrange multiplier $\gamma$ enforces the constraint on the classification loss.  

With applications in transfer learning, \citet{gao2020free} seek to evolve model parameters $\theta$ and the approximate posterior $q(\vz|\vx)$ along an `equilibrium surface' of optimal solutions to \eqref{eq:fep1}.  We interpret their free energy $F(\beta_D, \beta_C)$,  where $\beta_D, \beta_C$ are analogous to the \textit{intensive} variables of a physical system \cite{alemi2018therml}, as the negative log partition function $-\psi(\beta_D, \beta_C)$.  Written using the conjugate optimization \eqref{eq:conjugate} , we seek $\theta$, $q(\vz|\vx)$ yielding the appropriate distortion and classification loss $\eta_D, \eta_C$
\begin{align}
  -F(\beta_D, \beta_C)=  \psi(\beta_D, \beta_C) = \sup_{\eta_d,\eta_c} - \beta_D \, \eta_d - \beta_C \, \eta_c - \psi^{*}(\eta_d, \eta_c)  \label{eq:fe}
\end{align}
Similarly, for given moment constraints $\eta_D, \eta_C$, or \textit{extensive variables}, the optimal rate $R(D,C)$ corresponds to the conjugate $ \psi^{*}(\eta_D, \eta_C)$   %This fact ahs  which has not been explicitly observed in \cite{alemi2018therml, gao2020free}. 
\begin{align}
R(D,C) = \psi^{*}(\eta_D, \eta_C) = \sup \limits_{\beta_d, \beta_c } - \beta_d \, D - \beta_c \, C - \psi(\beta_d, \beta_c)
\label{eq:leg} 
\end{align}
At optimality on the `equilibrium surface' \cite{gao2020free}, we have $q(\vz|\vx) = \pi_{\beta}(\vz|\vx)$, which fulfills the constraints $\eta_{\beta} = \{ \eta_D, \eta_C \}$ for $\beta = \{ \beta_D, \beta_C \}$ and  the current decoder and classifier parameters $\theta$.   This corresponds to equality in the canonical Legendre duality equation \eqref{eq:legendre}
\begin{align}
 \psi^{*}(\eta_D, \eta_C) + \psi(\beta_D, \beta_C) - \beta_D \, \eta_D - \beta_C \, \eta_C = 0 \, . \label{eq:legendre_dc}
\end{align}
and also leads to the `first law of learning' from \cite{alemi2018therml} when $\psi(\beta_D, \beta_C)$ is considered as a fixed quantity.
%Interpreting the iso-classification constraint of \cite{gao2020free} and the partial Legendre transforms of \cite{alemi2018therml} using conjugate duality remains an interesting outstanding question.

==> sections/new_main/4_displaced_eq.tex <==

\section{Displaced Equilibrium} 
\begin{figure}
\includegraphics[width=.5\textwidth]{figs/rd_family.pdf}
\includegraphics[width=.5\textwidth]{figs/bercher_big.pdf}
\caption{Right: example with $\pi_0 = q(\vz)$}
\end{figure}
We now give an alternative interpretation of the Neyman-Pearson lemma in terms of thermodynamics.  \citet{bercher2012simple} consider a `displaced equilibrium' problem, where force is applied to displace an initial state $\pi_0$ by a given relative entropy $D_{KL}[\, r \, || \pi_0 ] = R$.  The system is then `attracted' toward a second distribution $\pi_1$ to obtain a new equilibrium.
\begin{align*}
     \mathcal{F}(R) = \min_{r} & \, D_{KL}[r(z) || \pi_1 (z)] \quad \text{subj. } \quad D_{KL}[r(z) || \pi_0 (z)] = R \\ 
     = \max \limits_{\lambda} \min \limits_{r} &  \, D_{KL}[r(z) || \pi_1 (z)] + \lambda \big( D_{KL}[r(z) || \pi_0 (z)] - R \big) \label{eq:fr}
\end{align*}
% \begin{align*}
%     \min_[r] D_{KL}[r(z) || \pi_1 (z)] \quad \text{subj. } \quad D_{KL}[r(z) || \pi_0 (z)] = R
% \end{align*}
As derived in \cref{app:fr_optimum}, the minimizing distribution $r^{*} = \argmin_r \mathcal{F}(R)$ has the form of a likelihood ratio exponential family \cite{brekelmans2019tvo}.
\begin{align*}
     r^{*}(z) &= \frac{\pi_0(z)^{\frac{\lambda}{1+\lambda}} \pi_1(z)^{\frac{1}{1+\lambda}}}{\int \pi_0(z)^{\frac{\lambda}{1+\lambda}} \pi_1(z)^{\frac{1}{1+\lambda}} dz} \\
\end{align*}
Letting $\frac{1}{1+\lambda} = \beta$  or $\lambda = \frac{1-\beta}{\beta} $, we obtain $r(z) \propto \pi_0(z)^{1-\beta} \pi_1(z)^{\beta}$. %where $\beta = \frac{1}{1+\lambda}$ is the Lagrange multiplier enforcing the constraint in \eqref{eq:fr}.  
Plugging this solution into the Lagrangian,
\begin{align*}
    \mathcal{F}(R) &= D_{KL}[\pi_{\beta}(z) || \pi_1 (z)] + \frac{1-\beta}{\beta} D_{KL}[\pi_{\beta}(z) || \pi_0 (z)] - \frac{1-\beta}{\beta} \, R \\
    &= \frac{1}{\beta} \bigg( \beta \, \psi (1) + (1-\beta) \, \psi (0) - \psi (\beta) \bigg) -  \frac{1-\beta}{\beta} \, R \\
     &= \frac{(1-\beta)}{\beta} \big(  D_{\beta}[\pi_1 || \pi_0 ] - \, R \big) 
\end{align*}
with $\psi (\beta)$ denoting the partition function .
% \footnote{Note, for distributions without a path exponential family \cite{brekelmans2019tvo}, we consider $D_{KL}[\pi_{\beta}(z) || \pi_1 (z)] = D_{\psi}[ \pi_1 (z) || \pi_{\beta}(z) ] = \psi_1 - \psi_{\beta} - (1-\beta) \eta_{\beta}$ with $\eta_{\beta} = \frac{\partial}{\partial \beta} \psi_{\beta}$.}
It can also be shown that the Renyi divergence between members of an exponential family corresponds to a gap in Jensen's inequality as above, so that $(1-\beta) D_{\beta}[\pi_1 || \pi_0] = \beta \, \psi (1) + (1-\beta) \, \psi (0) - \psi (\beta)$ \cite{nielsen2011r}.  Thus, minimization of $\mathcal{F}(R)$ amounts to minimizing a Renyi divergence, with order $\beta$ determined by the constraint value $R$.  \citet{bercher2012simple} also show that minimizing $\mathcal{F}(R)$ also corresponds to minimizing $D_{KL}[\pi_1 || \pi_{\beta}]$ or the symmetrized KL divergence  $D_{KL}^{\leftrightarrow}[\pi_1 ;  \pi_{0}]$ when the constraint is filled.


